Variability of the UV luminosity function with SPICE

We investigate the variability of the UV luminosity function (UVLF) at $z > 5$ using the SPICE suite of cosmological, radiation-hydrodynamic simulations, which include three distinct supernova (SN) feedback models: bursty-sn, smooth-sn, and hyper-sn. The bursty-sn model, driven by intense and episodic SN explosions, produces the highest fluctuations in the star formation rate (SFR). Conversely, the smooth-sn model, characterized by gentler SN feedback, results in minimal SFR variability. The hyper-sn model, featuring a more realistic prescription that incorporates hypernova (HN) explosions, exhibits intermediate variability, closely aligning with the smooth-sn trend at lower redshifts. These fluctuations in SFR significantly affect the $\rm{M_{UV} - M_{halo}}$ relation, a proxy for UVLF variability. Among the models, bursty-sn produces the highest UVLF variability, with a maximum value of 2.5. In contrast, the smooth-sn and hyper-sn models show substantially lower variability, with maximum values of 1.3 and 1.5, respectively. However, in all cases, UVLF variability strongly correlates with host halo mass, with lower-mass halos showing greater variability due to more effective SN feedback in their shallower gravitational wells. The bursty-sn model, though, results in higher amplitudes. Variability decreases in lower mass haloes with decreasing redshift for all feedback models. This study underscores the critical role of SN feedback in shaping the UVLF, and highlights the mass and redshift dependence of its variability, suggesting that UVLF variability may alleviate the bright galaxy tension observed by JWST at high redshifts.

==> xdm-errors <==
access control enabled, only authorized clients can connect
Warning: no access to tty (Inappropriate ioctl for device).
Thus no job control in this shell.
[1] 1568
egrep: warning: egrep is obsolescent; using grep -E
File Indexer suspended
Disabling and stopping the File Indexer
find: ‘/afs/mpa/home/basu/.local/share/applications’: No such file or directory
QObject: Cannot create children for a parent that is in a different thread.
(Parent is SplashApp(0x7ffebcb04e90), parent's thread is QThread(0x2042d40), current thread is QThread(0x20d0520)
QObject::installEventFilter(): Cannot filter events for objects in a different thread.
Connecting to deprecated signal QDBusConnectionInterface::serviceOwnerChanged(QString,QString,QString)
Initializing  "/afs/mpa/@sys/appl/kde-5.27.11_14.23/lib64/plugins/plasma/kcms/systemsettings/kcm_style.so"
Initializing  "/afs/mpa/@sys/appl/kde-5.27.11_14.23/lib64/plugins/plasma/kcms/systemsettings/kcm_fonts.so"
Initializing  "/afs/mpa/@sys/appl/kde-5.27.11_14.23/lib64/plugins/plasma/kcms/systemsettings/kcm_mouse.so"
org.kde.plasma.session: process job  "kcminit_startup" finished with exit code  0
kwin_xkbcommon: XKB: couldn't find a Compose file for locale "en_US.utf-8" (mapped to "en_US.utf-8")
Qt: Session management error: networkIdsList argument is NULL
Failed to write ice auth file entry
Failed to write xsmp ice auth file entry
Failed to write ice auth file entry
Failed to write xsmp ice auth file entry
Initializing  "/afs/mpa/@sys/appl/kde-5.27.11_14.23/lib64/plugins/plasma/kcms/systemsettings/kcm_touchpad.so"
kcm_touchpad: Using X11 backend
Initializing  "/afs/mpa/@sys/appl/kde-5.27.11_14.23/lib64/plugins/plasma/kcms/systemsettings/kcm_kgamma.so"
OpenGL vendor string:                   Intel
OpenGL renderer string:                 Mesa Intel(R) UHD Graphics 770 (ADL-S GT1)
OpenGL version string:                  4.6 (Compatibility Profile) Mesa 24.1.3
OpenGL shading language version string: 4.60
Driver:                                 Intel
GPU class:                              Unknown
OpenGL version:                         4.6
GLSL version:                           4.60
Mesa version:                           24.1.3
X server version:                       1.21.1
Linux kernel version:                   5.15.162
Requires strict binding:                yes
GLSL shaders:                           yes
Texture NPOT support:                   yes
Virtual Machine:                        no
Qt: Session management error: None of the authentication protocols specified are supported
Xlib XKB extension major= 1  minor= 0
kf.auth: Tried to start an invalid action:  "org.kde.powerdevil.discretegpuhelper.hasdualgpu"
Qt: Session management error: None of the authentication protocols specified are supported
org.kde.powerdevil: org.kde.powerdevil.discretegpuhelper.hasdualgpu failed
kf.i18n: KLocalizedString: Using an empty domain, fix the code. msgid: "kwrited" msgid_plural: "" msgctxt: ""
kf.auth: Tried to start an invalid action:  "org.kde.powerdevil.chargethresholdhelper.getthreshold"
org.kde.powerdevil: org.kde.powerdevil.chargethresholdhelper.getthreshold failed "Tried to start an invalid action"
kf.auth: Tried to start an invalid action:  "org.kde.powerdevil.backlighthelper.brightness"
org.kde.powerdevil: org.kde.powerdevil.backlighthelper.brightness failed
Qt: Session management error: None of the authentication protocols specified are supported
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
Qt: Session management error: None of the authentication protocols specified are supported
Qt: Session management error: None of the authentication protocols specified are supported
X server XKB extension major= 1  minor= 0
New PolkitAgentListener  0x7f0a58003da0
Adding new listener  PolkitQt1::Agent::Listener(0x7f0a3800c360) for  0x7f0a58003da0
Listener online
Authentication agent result: true
kf.auth: Tried to start an invalid action:  "org.kde.powerdevil.chargethresholdhelper.getthreshold"
org.kde.powerdevil: org.kde.powerdevil.chargethresholdhelper.getthreshold failed "Tried to start an invalid action"
org.kde.powerdevil: Handle button events action could not check for screen configuration
org.kde.powerdevil: The profile  "AC" tried to activate "DimDisplay" a non-existent action. This is usually due to an installation problem, a configuration problem, or because the action is not supported
QDBusConnection: name 'org.freedesktop.UDisks2' had owner '' but we thought it was ':1.18'
Installing the delayed initialization callback.
Failure: Module initialization failed
Aborting shell load: The activity manager daemon (kactivitymanagerd) is not running.
If this Plasma has been installed into a custom prefix, verify that its D-Bus services dir is known to the system for the daemon to be activatable.
Aborting shell load: The activity manager daemon (kactivitymanagerd) is not running.
If this Plasma has been installed into a custom prefix, verify that its D-Bus services dir is known to the system for the daemon to be activatable.
Qt: Session management error: None of the authentication protocols specified are supported
kf.plasma.quick: Applet preload policy set to 1
kcm_touchpad: Using X11 backend
Delayed initialization.
Reloading the khotkeys configuration
Version 2 File!
true
Imported file "/opt/kde-5.27.11_14.23/share/khotkeys/defaults.khotkeys"
Imported file "/opt/kde-5.27.11_14.23/share/khotkeys/kde32b1.khotkeys"
Imported file "/opt/kde-5.27.11_14.23/share/khotkeys/konqueror_gestures_kde321.khotkeys"
Known activities: ("fe916cd8-9d7d-4a11-9709-5fbae1e836c2")
QDBusAbstractAdaptor: Cannot relay signal KDEDModule::moduleDeleted(KDEDModule*): Pointers are not supported: KDEDModule*
kscreen.kded: UPower not available, lid detection won't work
10:24:00.689 › Logger Log level set to: info
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/lib64/qml/org/kde/kirigami.2/templates/InlineMessage.qml:265:13: QML SelectableLabel: Binding loop detected for property "implicitWidth"
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/lib64/qml/org/kde/kirigami.2/templates/InlineMessage.qml:265:13: QML SelectableLabel: Binding loop detected for property "implicitWidth"
10:24:00.891 › [App.Initialize] Current working directory is /afs/mpa/home/basu, changing into /afs/mpa/@sys/appl/mattermost-desktop-5.5.1
LaunchProcess: failed to execvp:
xdg-settings
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/wallpapers/org.kde.image/contents/ui/main.qml:20: TypeError: Cannot read property 'pluginName' of null
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/wallpapers/org.kde.image/contents/ui/main.qml:75: TypeError: Cannot read property 'configuration' of null
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/wallpapers/org.kde.image/contents/ui/main.qml:78: TypeError: Cannot read property 'pluginName' of null
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/wallpapers/org.kde.image/contents/ui/main.qml:80: TypeError: Cannot read property 'configuration' of null
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/wallpapers/org.kde.image/contents/ui/main.qml:81: TypeError: Cannot read property 'configuration' of null
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/wallpapers/org.kde.image/contents/ui/main.qml:82: TypeError: Cannot read property 'configuration' of null
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/wallpapers/org.kde.image/contents/ui/main.qml:83: TypeError: Cannot read property 'configuration' of null
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/wallpapers/org.kde.image/contents/ui/main.qml:84: TypeError: Cannot read property 'configuration' of null
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/wallpapers/org.kde.image/contents/ui/main.qml:16: TypeError: Cannot read property 'configuration' of null
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/wallpapers/org.kde.image/contents/ui/main.qml:17: TypeError: Cannot read property 'configuration' of null
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/wallpapers/org.kde.image/contents/ui/main.qml:18: TypeError: Cannot read property 'configuration' of null
QObject::connect: No such slot DesktopProtocol::_k_slotRedirection(KIO::Job *, QUrl)
Gtk-Message: 10:24:01.031: Failed to load module "colorreload-gtk-module"
Gtk-Message: 10:24:01.031: Failed to load module "window-decorations-gtk-module"
kwin_core: XCB error: 150 (BadDamage), sequence: 3227, resource id: 23068720, major code: 142 (DAMAGE), minor code: 3 (Subtract)
10:24:01.195 › [App.Config] config.autostart has been configured: true
10:24:01.261 › [App.Initialize] Autoupgrade disabled: false
10:24:01.532 › [ServerDropdownView] init
10:24:01.545 › [i18nManager] Failed to set new language en-US
10:24:01.554 › [i18nManager] Failed to set new language US
Trying to use rootObject before initialization is completed, whilst using setInitializationDelayed. Forcing completion
org.kde.plasma.kicker: Entry is not valid "ktp-contactlist.desktop" QSharedPointer(0x1faaa80)
org.kde.plasma.kicker: Entry is not valid "org.kde.discover.desktop" QSharedPointer(0x1fa9a60)
org.kde.plasma.kicker: Entry is not valid "ktp-contactlist.desktop" QSharedPointer(0x1faba20)
org.kde.plasma.kicker: Entry is not valid "org.kde.discover.desktop" QSharedPointer(0x1fab510)
Registering ":1.31/StatusNotifierItem" to system tray
10:24:01.825 › [App.Config] config.autostart has been configured: true
Cyclic dependency detected between "file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml" and "file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/NotificationHeader.qml"
Cyclic dependency detected between "file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml" and "file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/ThumbnailStrip.qml"
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
10:24:02.397 › [App.Config] config.autostart has been configured: true
QFont::setPointSizeF: Point size <= 0 (0.000000), must be greater than 0
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.battery/contents/ui/CompactRepresentation.qml:61:17: Unable to assign [undefined] to int
org.kde.plasma.pulseaudio: No object for name "alsa_output.pci-0000_00_1f.3.analog-stereo.monitor"
Service  ":1.31" unregistered
kwin_core: XCB error: 150 (BadDamage), sequence: 7410, resource id: 23068718, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Gtk-Message: 10:24:13.268: Failed to load module "colorreload-gtk-module"
Gtk-Message: 10:24:13.268: Failed to load module "window-decorations-gtk-module"
[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'blocklist.mlbf_source' into metrics: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'blocklist.mlbf_generation_time' into metrics: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'blocklist.mlbf_stash_time_oldest' into metrics: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'blocklist.mlbf_stash_time_newest' into metrics: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'blocklist.last_modified_rs_addons_mblf' into metrics: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[Parent 2199, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:2199): WARNING **: 10:31:09.072: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/lib64/qml/org/kde/plasma/extras/PlaceholderMessage.qml:238:5: QML Heading: Binding loop detected for property "verticalAlignment"
qt.xkb.compose: failed to create compose table
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/contacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/contacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/emailContacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/emailContacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/contacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/emailContacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/contacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/emailContacts/"
kf.config.core: couldn't lock local file
10:41:29.431 › Logger Log level set to: info
10:41:29.502 › [App.Initialize] Current working directory is /afs/mpa/home/basu, changing into /afs/mpa/@sys/appl/mattermost-desktop-5.5.1
[3746:1018/104129.506097:ERROR:process_singleton_posix.cc(339)] Failed to create /afs/mpa/home/basu/.config/Mattermost/SingletonLock: Disk quota exceeded (122)
kf.config.core: couldn't lock local file
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/lib64/qml/org/kde/plasma/extras/PlaceholderMessage.qml:238:5: QML Heading: Binding loop detected for property "verticalAlignment"
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/lib64/qml/org/kde/plasma/extras/PlaceholderMessage.qml:238:5: QML Heading: Binding loop detected for property "verticalAlignment"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/contacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/emailContacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/contacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/emailContacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/contacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/emailContacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/contacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/emailContacts/"
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
10:41:38.632 › Logger Log level set to: info
10:41:38.703 › [App.Initialize] Current working directory is /afs/mpa/home/basu, changing into /afs/mpa/@sys/appl/mattermost-desktop-5.5.1
[3790:1018/104138.706561:ERROR:process_singleton_posix.cc(339)] Failed to create /afs/mpa/home/basu/.config/Mattermost/SingletonLock: Disk quota exceeded (122)
trying to show an empty dialog
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
kwin_core: XCB error: 3 (BadWindow), sequence: 60159, resource id: 33554446, major code: 129 (SHAPE), minor code: 6 (Input)
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/lib64/qml/org/kde/plasma/extras/PlaceholderMessage.qml:238:5: QML Heading: Binding loop detected for property "verticalAlignment"
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
kwin_core: XCB error: 3 (BadWindow), sequence: 33588, resource id: 33554453, major code: 129 (SHAPE), minor code: 6 (Input)
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[Parent 2199, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:2199): WARNING **: 14:02:53.389: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[GFX1-]: RenderCompositorSWGL failed mapping default framebuffer, no dt
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'pageload#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'pageload#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'blocklist.mlbf_source' into metrics: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'blocklist.mlbf_generation_time' into metrics: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'blocklist.mlbf_stash_time_oldest' into metrics: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'blocklist.mlbf_stash_time_newest' into metrics: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'blocklist.last_modified_rs_addons_mblf' into metrics: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
[ERROR glean_core::database] Failed to record metric 'disable-ads-startup-cache#experiment' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab-topic-labels#experiment' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'pdf-annotations-highlight-already-default-handler-v2#experiment' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'disabling-chips-for-v131#experiment' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::metrics::experiment] Failed to set experiment as inactive: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
kwin_core: XCB error: 3 (BadWindow), sequence: 52157, resource id: 33554459, major code: 129 (SHAPE), minor code: 6 (Input)
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
[ERROR glean_core::database] Failed to record metric 'blocklist.mlbf_source' into metrics: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'blocklist.mlbf_generation_time' into metrics: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'blocklist.mlbf_stash_time_oldest' into metrics: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'blocklist.mlbf_stash_time_newest' into metrics: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'blocklist.last_modified_rs_addons_mblf' into metrics: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'metrics#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'metrics#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'mps.last_sent_time' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
kwin_core: XCB error: 3 (BadWindow), sequence: 59540, resource id: 33554465, major code: 129 (SHAPE), minor code: 6 (Input)
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'pageload#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'pageload#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[Parent 2199, Unnamed thread 7f8bc95f1700] WARNING: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.GXV6V2”: Disk quota exceeded: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

(firefox:2199): dconf-WARNING **: 15:24:33.584: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.GXV6V2”: Disk quota exceeded
[Parent 2199, Main Thread] WARNING: Attempting to store changes into '/afs/mpa/home/basu/.local/share/recently-used.xbel', but failed: Failed to create file “/afs/mpa/home/basu/.local/share/recently-used.xbel.20R6V2”: Disk quota exceeded: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

(firefox:2199): Gtk-WARNING **: 15:24:33.587: Attempting to store changes into '/afs/mpa/home/basu/.local/share/recently-used.xbel', but failed: Failed to create file “/afs/mpa/home/basu/.local/share/recently-used.xbel.20R6V2”: Disk quota exceeded
[Parent 2199, Unnamed thread 7f8bc95f1700] WARNING: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.MF4XV2”: Disk quota exceeded: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

(firefox:2199): dconf-WARNING **: 15:24:36.438: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.MF4XV2”: Disk quota exceeded
Qt: Session management error: None of the authentication protocols specified are supported
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.taskmanager/contents/ui/Task.qml:286: Unable to assign [undefined] to QString
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
kf.kio.widgets: Cannot read information about filesystem under path "/var/tmp/xdgcache-basu/thumbnails/"
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
kwin_core: XCB error: 3 (BadWindow), sequence: 29409, resource id: 33554473, major code: 129 (SHAPE), minor code: 6 (Input)
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
kf.kio.core: Failed to lock recently used
kf.kio.core: Failed to add to recently used bookmark file
kf.config.core: couldn't lock local file
Qt: Session management error: None of the authentication protocols specified are supported
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
kwin_core: XCB error: 150 (BadDamage), sequence: 55993, resource id: 23217913, major code: 142 (DAMAGE), minor code: 3 (Subtract)
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
Cannot initialize model with data QJsonObject(). missing: QJsonValue(string, "urls")
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
"Could not write to file /afs/mpa/home/basu/.local/share/Trash/info/application_Garaldi (1).pdf.trashinfo."
kwin_core: XCB error: 150 (BadDamage), sequence: 59448, resource id: 23218221, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Qt: Session management error: None of the authentication protocols specified are supported
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.taskmanager/contents/ui/Task.qml:286: Unable to assign [undefined] to QString
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
qt.xkb.compose: failed to create compose table
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
Qt: Session management error: None of the authentication protocols specified are supported
kf.i18n.kuit: "Unknown subcue ':whatsthis,' in UI marker in context {@info:whatsthis, %1 the action's text}."
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/qoi"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-aptus-mos"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-arq"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-bay"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-bmq"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-cap"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-cine"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-cs1"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-dc2"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-drf"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-dxo"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-epson-eip"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-epson-erf"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-fff"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-hasselblad-3fr"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-iiq"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-kodak-dcs"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-kodak-kc2"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-mamiya-mef"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-mfw"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-minolta-mdc"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-mng"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-obm"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-ori"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-ptx"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-pxn"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-qtk"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-r3d"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-raw"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-rdc"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-rwl"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-rwz"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-samsung-srw"
org.kde.kdegraphics.gwenview.lib: Unresolved mime type  "image/x-sti"
org.kde.kdegraphics.gwenview.lib: Unresolved raw mime type  "image/x-samsung-srw"
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/lib64/qml/org/kde/plasma/extras/PlaceholderMessage.qml:238:5: QML Heading: Binding loop detected for property "verticalAlignment"
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/lib64/qml/org/kde/plasma/extras/PlaceholderMessage.qml:238:5: QML Heading: Binding loop detected for property "verticalAlignment"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/contacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/emailContacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/contacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/emailContacts/"
18:34:03.258 › Logger Log level set to: info
18:34:03.335 › [App.Initialize] Current working directory is /afs/mpa/home/basu, changing into /afs/mpa/@sys/appl/mattermost-desktop-5.5.1
LaunchProcess: failed to execvp:
xdg-settings
Gtk-Message: 18:34:03.363: Failed to load module "colorreload-gtk-module"
Gtk-Message: 18:34:03.363: Failed to load module "window-decorations-gtk-module"
18:34:03.374 › [App.Config] config.autostart has been configured: true
18:34:03.384 › [App.Initialize] Autoupgrade disabled: false
18:34:03.412 › [ServerDropdownView] init
18:34:03.421 › [i18nManager] Failed to set new language en-US
18:34:03.424 › [i18nManager] Failed to set new language US
18:34:03.442 › [App.Config] config.autostart has been configured: true
Registering ":1.68/StatusNotifierItem" to system tray
18:34:03.855 › [App.Config] config.autostart has been configured: true
[4579:1019/183424.656501:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[4637:1019/183435.706017:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file

(mattermost-desktop:4579): dconf-WARNING **: 18:34:48.937: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.PK09V2”: Disk quota exceeded

(mattermost-desktop:4579): dconf-WARNING **: 18:34:48.955: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.KAM9V2”: Disk quota exceeded

(mattermost-desktop:4579): dconf-WARNING **: 18:34:50.488: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.58HXV2”: Disk quota exceeded

(mattermost-desktop:4579): dconf-WARNING **: 18:34:51.868: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.ZMUBW2”: Disk quota exceeded

(mattermost-desktop:4579): dconf-WARNING **: 18:34:51.868: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.Q6TBW2”: Disk quota exceeded

(mattermost-desktop:4579): Gtk-WARNING **: 18:34:52.120: Attempting to store changes into '/afs/mpa/home/basu/.local/share/recently-used.xbel', but failed: Failed to create file “/afs/mpa/home/basu/.local/share/recently-used.xbel.6USTV2”: Disk quota exceeded

(mattermost-desktop:4579): dconf-WARNING **: 18:34:56.244: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.CCIRV2”: Disk quota exceeded

(mattermost-desktop:4579): dconf-WARNING **: 18:34:56.275: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.2Z21V2”: Disk quota exceeded

(mattermost-desktop:4579): dconf-WARNING **: 18:34:56.295: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.FQA1V2”: Disk quota exceeded

(mattermost-desktop:4579): dconf-WARNING **: 18:34:57.957: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.D5K9V2”: Disk quota exceeded

(mattermost-desktop:4579): dconf-WARNING **: 18:34:58.121: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.2TSTV2”: Disk quota exceeded

(mattermost-desktop:4579): dconf-WARNING **: 18:34:58.765: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.G8S2V2”: Disk quota exceeded
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }

(mattermost-desktop:4579): dconf-WARNING **: 18:34:59.512: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.3HNWV2”: Disk quota exceeded

(mattermost-desktop:4579): dconf-WARNING **: 18:34:59.894: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.JOABW2”: Disk quota exceeded

(mattermost-desktop:4579): dconf-WARNING **: 18:35:01.534: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.MPR7V2”: Disk quota exceeded

(mattermost-desktop:4579): dconf-WARNING **: 18:35:06.364: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.EHTZV2”: Disk quota exceeded

(mattermost-desktop:4579): dconf-WARNING **: 18:35:06.365: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.2USZV2”: Disk quota exceeded

(mattermost-desktop:4579): Gtk-WARNING **: 18:35:06.619: Attempting to store changes into '/afs/mpa/home/basu/.local/share/recently-used.xbel', but failed: Failed to create file “/afs/mpa/home/basu/.local/share/recently-used.xbel.FUX5V2”: Disk quota exceeded
[4579:1019/183531.619359:ERROR:indexed_db_backing_store.cc(3468)] IndexedDB Write Error: TRANSACTION_COMMIT_METHOD
[4579:1019/183532.806520:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[4637:1019/183532.889866:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[4579:1019/183534.408076:ERROR:indexed_db_backing_store.cc(3468)] IndexedDB Write Error: TRANSACTION_COMMIT_METHOD
[4579:1019/183535.908700:ERROR:indexed_db_backing_store.cc(3468)] IndexedDB Write Error: TRANSACTION_COMMIT_METHOD
[4579:1019/183538.231717:ERROR:indexed_db_backing_store.cc(3468)] IndexedDB Write Error: TRANSACTION_COMMIT_METHOD
[4579:1019/183540.541651:ERROR:indexed_db_backing_store.cc(3468)] IndexedDB Write Error: TRANSACTION_COMMIT_METHOD
[4637:1019/183614.017686:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
[ERROR glean_core::database] Failed to record metric 'metrics#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'metrics#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'mps.last_sent_time' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[4637:1020/153637.124303:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
LaunchProcess: failed to execvp:
xdg-open
LaunchProcess: failed to execvp:
xdg-open
LaunchProcess: failed to execvp:
xdg-open
kwin_core: XCB error: 3 (BadWindow), sequence: 29337, resource id: 69206051, major code: 129 (SHAPE), minor code: 6 (Input)
[Parent 2199, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:2199): WARNING **: 20:18:35.804: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

libva info: VA-API version 1.22.0
libva info: Trying to open /usr/lib64/dri/iHD_drv_video.so
libva info: Found init function __vaDriverInit_1_22
libva info: va_openDriver() returns 0
Gtk-Message: 20:22:27.230: Failed to load module "colorreload-gtk-module"
Gtk-Message: 20:22:27.230: Failed to load module "window-decorations-gtk-module"
[Parent 2199, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:2199): WARNING **: 20:45:40.817: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

Missing chrome or resource URL: chrome://browser/skin/aboutSessionRestore-window-icon.png
Missing chrome or resource URL: chrome://browser/skin/abyss/img/waterfox-abyss-preview.svg
[Parent 2199, Main Thread] WARNING: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.Avahi was not provided by any .service files: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:2199): WARNING **: 21:01:36.838: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.Avahi was not provided by any .service files
[Parent 2199, Main Thread] WARNING: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.Avahi was not provided by any .service files: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:2199): WARNING **: 21:01:36.838: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.Avahi was not provided by any .service files
kwin_core: XCB error: 150 (BadDamage), sequence: 705, resource id: 23069545, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Service  ":1.68" unregistered
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/lib64/qml/org/kde/plasma/extras/PlaceholderMessage.qml:238:5: QML Heading: Binding loop detected for property "verticalAlignment"
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.taskmanager/contents/ui/Task.qml:286: Unable to assign [undefined] to QString
Gtk-Message: 13:48:05.163: Failed to load module "colorreload-gtk-module"
Gtk-Message: 13:48:05.163: Failed to load module "window-decorations-gtk-module"
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/lib64/qml/org/kde/plasma/extras/PlaceholderMessage.qml:238:5: QML Heading: Binding loop detected for property "verticalAlignment"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/contacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/emailContacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/contacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/emailContacts/"
14:10:22.727 › Logger Log level set to: info
14:10:22.805 › [App.Initialize] Current working directory is /afs/mpa/home/basu, changing into /afs/mpa/@sys/appl/mattermost-desktop-5.5.1
LaunchProcess: failed to execvp:
xdg-settings
Gtk-Message: 14:10:22.827: Failed to load module "colorreload-gtk-module"
Gtk-Message: 14:10:22.827: Failed to load module "window-decorations-gtk-module"
14:10:22.836 › [App.Config] config.autostart has been configured: true
14:10:22.845 › [App.Initialize] Autoupgrade disabled: false
14:10:22.874 › [ServerDropdownView] init
14:10:22.887 › [i18nManager] Failed to set new language en-US
14:10:22.889 › [i18nManager] Failed to set new language US
14:10:22.907 › [App.Config] config.autostart has been configured: true
Registering ":1.83/StatusNotifierItem" to system tray
14:10:23.289 › [App.Config] config.autostart has been configured: true
14:16:25.128 › [Notifications] notification not supported
14:25:28.881 › [Notifications] notification not supported
14:25:37.209 › [Notifications] notification not supported
14:25:37.992 › [Notifications] notification not supported
14:25:50.877 › [Notifications] notification not supported
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
[Parent 9747, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:9747): WARNING **: 10:33:07.642: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
LaunchProcess: failed to execvp:
xdg-open
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
kwin_core: XCB error: 3 (BadWindow), sequence: 19225, resource id: 33554510, major code: 129 (SHAPE), minor code: 6 (Input)
Qt: Session management error: None of the authentication protocols specified are supported
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.taskmanager/contents/ui/Task.qml:286: Unable to assign [undefined] to QString
qt.xkb.compose: failed to create compose table
kwin_core: XCB error: 150 (BadDamage), sequence: 44910, resource id: 23335991, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
kwin_core: XCB error: 3 (BadWindow), sequence: 8889, resource id: 6293312, major code: 129 (SHAPE), minor code: 6 (Input)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x30c79c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x30c79c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 53, resource id: 23390597, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x20b1480) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x20b1480) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 5966, resource id: 23391206, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x20b1480) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x20b1480) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1059df0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1059df0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 15507, resource id: 23392100, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5e9c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5e9c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x121c160) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x121c160) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 25172, resource id: 23392917, major code: 142 (DAMAGE), minor code: 3 (Subtract)
kwin_core: Failed to focus 0x4a0021b (error 3)
kwin_core: XCB error: 3 (BadWindow), sequence: 26139, resource id: 77595163, major code: 129 (SHAPE), minor code: 3 (Combine)
kwin_core: XCB error: 3 (BadWindow), sequence: 26140, resource id: 77595163, major code: 129 (SHAPE), minor code: 3 (Combine)
kwin_core: XCB error: 3 (BadWindow), sequence: 26159, resource id: 77595163, major code: 129 (SHAPE), minor code: 3 (Combine)
kwin_core: XCB error: 3 (BadWindow), sequence: 26160, resource id: 77595163, major code: 129 (SHAPE), minor code: 3 (Combine)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2202480) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2202480) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11817b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11817b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x23fd9b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x23fd9b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1152ce0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1152ce0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 53469, resource id: 23395730, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4115b70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4115b70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 60782, resource id: 23396519, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f52f20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f52f20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 2606, resource id: 23397307, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2aaada0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2aaada0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fe8e10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fe8e10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 19260, resource id: 23399045, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fe4910) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fe4910) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 27018, resource id: 23399809, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e96890) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e96890) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 35493, resource id: 23400752, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d848d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d848d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 43556, resource id: 23401540, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11bd110) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11bd110) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 51395, resource id: 23402441, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fc8200) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fc8200) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 58462, resource id: 23403243, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4157fb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4157fb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f3fa015b3d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f3fa015b3d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 7778, resource id: 23404787, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9a30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9a30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 13422, resource id: 23405462, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33471f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33471f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d6f6e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d6f6e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 27047, resource id: 23406868, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2efa9b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2efa9b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 34619, resource id: 23407676, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f4144019a90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f4144019a90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 41477, resource id: 23408380, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e991c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e991c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 47254, resource id: 23409111, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dd0850) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dd0850) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x305b470) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x305b470) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 894, resource id: 23410794, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x412e870) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x412e870) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 9562, resource id: 23411717, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3739490) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3739490) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 19308, resource id: 23412645, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d520f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d520f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fb0650) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fb0650) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 37814, resource id: 23414633, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d520f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d520f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 46082, resource id: 23415584, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3364d30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3364d30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 53664, resource id: 23416433, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a65e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a65e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 61373, resource id: 23417235, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x24a2d30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x24a2d30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 5382, resource id: 23418334, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12a4bc0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12a4bc0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 14657, resource id: 23419316, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dcd580) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dcd580) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1126320) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1126320) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9c9a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9c9a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x24a2d40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x24a2d40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 46860, resource id: 23422968, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f19ae0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f19ae0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed4620) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed4620) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x305c420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x305c420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 65385, resource id: 23424946, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e88910) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e88910) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 6030, resource id: 23425587, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x305c420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x305c420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 14673, resource id: 23426367, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a41690) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a41690) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f4144025ec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f4144025ec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 31728, resource id: 23428264, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12d8d20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12d8d20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 41138, resource id: 23429187, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f4144025ec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f4144025ec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 49988, resource id: 23430140, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9e7d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9e7d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 57897, resource id: 23430986, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3054d40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3054d40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 981, resource id: 23431974, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f84bb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f84bb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 9536, resource id: 23432916, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x20afb10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x20afb10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 16196, resource id: 23433655, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fada00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fada00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 23268, resource id: 23434338, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9bf90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9bf90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 30072, resource id: 23435064, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4102c90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4102c90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 36599, resource id: 23435726, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a6030) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a6030) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9e7d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9e7d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 50069, resource id: 23437095, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x121ca40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x121ca40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 57289, resource id: 23437851, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea3af0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea3af0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 65135, resource id: 23438603, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x30b8980) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x30b8980) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f52190) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f52190) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 15117, resource id: 23440320, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1294850) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1294850) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 22326, resource id: 23441080, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f4b410) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f4b410) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 30195, resource id: 23441925, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x22064d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x22064d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 37086, resource id: 23442660, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc7d90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc7d90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 45052, resource id: 23443479, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d84900) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d84900) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 51189, resource id: 23444157, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e90150) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e90150) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e71a40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e71a40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 63881, resource id: 23445397, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x128af50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x128af50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 5224, resource id: 23446223, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb0600) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb0600) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 11876, resource id: 23446801, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9180) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9180) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 18326, resource id: 23447563, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x128af50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x128af50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9f7a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9f7a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 29512, resource id: 23448681, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e91bb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e91bb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 35734, resource id: 23449338, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x15f88e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x15f88e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 42649, resource id: 23450015, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fce8a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fce8a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12a6720) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12a6720) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f2bab0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f2bab0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 3166, resource id: 23452907, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x308b490) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x308b490) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fc46b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fc46b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 18437, resource id: 23454355, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x410f6b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x410f6b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 27321, resource id: 23455302, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f04fb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f04fb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2ce66d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2ce66d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 41620, resource id: 23457093, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed11e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed11e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 50411, resource id: 23457696, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10f9b70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10f9b70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 59505, resource id: 23458754, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f2c430) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f2c430) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 2371, resource id: 23459655, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35c03b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35c03b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 11554, resource id: 23460643, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x308b490) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x308b490) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 17827, resource id: 23461374, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3610a40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3610a40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 26228, resource id: 23462305, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f47c60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f47c60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3610a40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3610a40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1264870) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1264870) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 52061, resource id: 23464980, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ebdd30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ebdd30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 60599, resource id: 23465873, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1296bf0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1296bf0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 3893, resource id: 23466759, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9f230) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9f230) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb43c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb43c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 21030, resource id: 23468531, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea85b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea85b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 28487, resource id: 23469358, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e6e260) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e6e260) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 35716, resource id: 23470192, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e8d1c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e8d1c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b310) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b310) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 50179, resource id: 23471639, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1099080) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1099080) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 58328, resource id: 23472438, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4129c20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4129c20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed18f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed18f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1065190) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1065190) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 18009, resource id: 23475257, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10c3de0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10c3de0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 26305, resource id: 23476174, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f29b00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f29b00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x339e080) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x339e080) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1275650) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1275650) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 49022, resource id: 23478522, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2ab4680) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2ab4680) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 57261, resource id: 23479388, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4109500) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4109500) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 64997, resource id: 23480226, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1153b80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1153b80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x122b520) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x122b520) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 15141, resource id: 23481820, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eae900) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eae900) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 22911, resource id: 23482624, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9a9d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9a9d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x412edd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x412edd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 39265, resource id: 23484339, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9a9d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9a9d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 46802, resource id: 23485146, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fc8e70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fc8e70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f33990) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f33990) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 62071, resource id: 23486749, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e91a10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e91a10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 4578, resource id: 23487604, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115c150) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115c150) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 11971, resource id: 23488380, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x26c3cc0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x26c3cc0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 19938, resource id: 23489183, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x32f6e50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x32f6e50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3056e90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3056e90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 35644, resource id: 23490903, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed0ae0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed0ae0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 43937, resource id: 23491777, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35eaf10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35eaf10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 52017, resource id: 23492580, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fe13e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fe13e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 59964, resource id: 23493536, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fdbd30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fdbd30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 2116, resource id: 23494295, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e90b10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e90b10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 9641, resource id: 23495171, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f7d1f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f7d1f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 17774, resource id: 23496048, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea95a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea95a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f7d1f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f7d1f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 33362, resource id: 23497705, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f7d1f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f7d1f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 39832, resource id: 23498391, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fdb3a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fdb3a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3380b00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3380b00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12b9970) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12b9970) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 65185, resource id: 23501054, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fe96c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fe96c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 10426, resource id: 23502098, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x236ac40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x236ac40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed47f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed47f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3380b00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3380b00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 37981, resource id: 23505636, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e90060) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e90060) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 45024, resource id: 23506427, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dd1850) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dd1850) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fe0d70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fe0d70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e86340) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e86340) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a83e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a83e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 10684, resource id: 23509846, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33611a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33611a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a83e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a83e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33611a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33611a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 35401, resource id: 23512384, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12d6580) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12d6580) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 43360, resource id: 23513246, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e87aa0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e87aa0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 51589, resource id: 23514070, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f7e320) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f7e320) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3611e80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3611e80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 1881, resource id: 23515742, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e667f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e667f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 9907, resource id: 23516679, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21e0490) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21e0490) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed4290) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed4290) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 26045, resource id: 23518342, major code: 142 (DAMAGE), minor code: 3 (Subtract)
[GFX1-]: RenderCompositorSWGL failed mapping default framebuffer, no dt
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e92a70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e92a70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 34130, resource id: 23519130, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed4290) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed4290) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fdee20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fdee20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dd2f60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dd2f60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 60992, resource id: 23522503, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f51f40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f51f40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 5946, resource id: 23523635, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dd2f60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dd2f60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x23156b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x23156b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f71bb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f71bb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 29071, resource id: 23526060, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1295b90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1295b90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 36743, resource id: 23526959, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f68a30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f68a30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x23156b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x23156b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10fa130) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10fa130) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 61016, resource id: 23529566, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb5380) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb5380) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 2318, resource id: 23530343, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x23156b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x23156b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb1f70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb1f70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 18720, resource id: 23532173, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fd0660) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fd0660) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 29757, resource id: 23533005, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb1f70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb1f70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 36467, resource id: 23533894, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c78910) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c78910) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e68690) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e68690) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c78910) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c78910) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 58853, resource id: 23536231, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f68a30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f68a30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 1575, resource id: 23537157, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2c52c60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2c52c60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 11259, resource id: 23538168, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a4a750) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a4a750) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1cbabc0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1cbabc0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 32678, resource id: 23540448, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33474f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33474f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12479e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12479e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 51027, resource id: 23542931, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dd24c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dd24c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33dde30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33dde30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 666, resource id: 23544621, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f27720) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f27720) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 6630, resource id: 23545322, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f43160) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f43160) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea67c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea67c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e61470) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e61470) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 31065, resource id: 23547817, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fc5ac0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fc5ac0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 39720, resource id: 23548768, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f17d50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f17d50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fc5ac0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fc5ac0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 53538, resource id: 23550247, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb5a30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb5a30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 60991, resource id: 23551030, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fc7c40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fc7c40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 2947, resource id: 23551787, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12241c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12241c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 10141, resource id: 23552647, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12bf300) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12bf300) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 17399, resource id: 23553419, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dce540) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dce540) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 26320, resource id: 23554281, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3347240) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3347240) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 35357, resource id: 23555096, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x336b5a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x336b5a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f3fc81d3540) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f3fc81d3540) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 51573, resource id: 23557259, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x24a2430) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x24a2430) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2261860) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2261860) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fafb80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fafb80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f3fc81d3540) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f3fc81d3540) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 20701, resource id: 23561196, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9f340) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9f340) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 27401, resource id: 23562020, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x412c7b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x412c7b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9f340) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9f340) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ead7a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ead7a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 47854, resource id: 23564091, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb2250) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb2250) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 53190, resource id: 23564734, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9f340) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9f340) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11bd110) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11bd110) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11bd110) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11bd110) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 3580, resource id: 23566342, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x24df150) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x24df150) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 8756, resource id: 23566860, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x126e690) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x126e690) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 14115, resource id: 23567395, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb95a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb95a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9d0e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9d0e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 24824, resource id: 23568468, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb74e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb74e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 30234, resource id: 23569030, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f2de30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f2de30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10cd170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10cd170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41045d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41045d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 51195, resource id: 23571064, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fada70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fada70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 56927, resource id: 23571736, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41045d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41045d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 62828, resource id: 23572324, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3338ae0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3338ae0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 5341, resource id: 23573022, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2245120) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2245120) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 12314, resource id: 23573824, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f328f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f328f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 18561, resource id: 23574426, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2ff80f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2ff80f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 27454, resource id: 23575280, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1093a90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1093a90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4154310) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4154310) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 43656, resource id: 23576949, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35eb030) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35eb030) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 48717, resource id: 23577568, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33313c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33313c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9c340) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9c340) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12648a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12648a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 8563, resource id: 23579927, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e68340) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e68340) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 15017, resource id: 23580735, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed4290) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed4290) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 21316, resource id: 23581371, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x412f000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x412f000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e82be0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e82be0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 34013, resource id: 23582684, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb0390) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb0390) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 42619, resource id: 23583549, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x30919d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x30919d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb4330) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb4330) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fd1b10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fd1b10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 60983, resource id: 23585502, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x412c970) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x412c970) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 3638, resource id: 23586392, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42b1dd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42b1dd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e86d90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e86d90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1097b30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1097b30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 23079, resource id: 23588446, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed4210) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed4210) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 28680, resource id: 23589112, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x308c9e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x308c9e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb1240) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb1240) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 42932, resource id: 23590588, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x24a9470) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x24a9470) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 48600, resource id: 23591217, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34a8370) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34a8370) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9d120) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9d120) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 61330, resource id: 23592430, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c78ca0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c78ca0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 2824, resource id: 23593251, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9d120) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9d120) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 8306, resource id: 23593797, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ead7a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ead7a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 15761, resource id: 23594463, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33bf7e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33bf7e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 24264, resource id: 23595346, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12713f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12713f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 33453, resource id: 23596414, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c99850) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c99850) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 40942, resource id: 23597233, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33474f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33474f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3cab640) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3cab640) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 57112, resource id: 23598724, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33474f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33474f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 146, resource id: 23599581, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f3fe41fd3b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f3fe41fd3b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 8779, resource id: 23600545, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d91bb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d91bb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 15829, resource id: 23601392, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3cab640) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3cab640) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 21144, resource id: 23601923, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e96770) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e96770) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 26448, resource id: 23602454, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e88e00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e88e00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f414401dcc0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f414401dcc0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 43674, resource id: 23604003, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e4600) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e4600) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x105c3f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x105c3f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 60975, resource id: 23605834, major code: 142 (DAMAGE), minor code: 3 (Subtract)
[Parent 9747, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:9747): WARNING **: 17:47:13.172: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fcf630) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fcf630) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 3832, resource id: 23606635, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb2ae0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb2ae0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f1bec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f1bec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dd2520) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dd2520) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 29234, resource id: 23609233, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x122e0e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x122e0e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")

malloc: unknown:0: assertion botched
free: start and end chunk sizes differ
Aborting...
malloc: unknown:0: assertion botched
free: start and end chunk sizes differ
Aborting...kwin_core: XCB error: 150 (BadDamage), sequence: 37875, resource id: 23610034, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b6e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b6e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 46091, resource id: 23610875, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x285d4f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x285d4f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42b1920) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42b1920) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 63277, resource id: 23612471, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34a31c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34a31c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 6135, resource id: 23613423, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e8e670) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e8e670) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e8cf00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e8cf00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e8e670) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e8e670) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 30100, resource id: 23616151, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1250530) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1250530) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 35761, resource id: 23616723, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2245120) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2245120) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33da2f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33da2f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 46921, resource id: 23617847, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1051d70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1051d70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 52565, resource id: 23618423, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f2e010) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f2e010) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 57571, resource id: 23618902, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2323f40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2323f40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 63124, resource id: 23619467, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x272bc80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x272bc80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 3171, resource id: 23620024, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1158e10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1158e10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 8741, resource id: 23620588, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9a990) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9a990) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 14351, resource id: 23621154, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3feb050) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3feb050) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 19928, resource id: 23621719, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1062b50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1062b50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 25612, resource id: 23622291, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e96620) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e96620) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 31295, resource id: 23622873, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e5d950) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e5d950) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 37021, resource id: 23623456, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fada40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fada40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 42700, resource id: 23624041, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e5d950) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e5d950) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 48274, resource id: 23624604, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff7f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff7f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 53853, resource id: 23625170, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2232f00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2232f00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 59430, resource id: 23625733, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f56940) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f56940) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x37118a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x37118a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 5376, resource id: 23626904, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e88030) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e88030) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 10948, resource id: 23627467, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c999b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c999b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 16562, resource id: 23628037, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e96a90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e96a90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f1aa10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f1aa10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 27654, resource id: 23629156, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9fdf0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9fdf0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 33262, resource id: 23629714, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f209f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f209f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 38801, resource id: 23630278, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e86280) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e86280) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f13290) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f13290) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 49945, resource id: 23631397, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e1f70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e1f70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 55597, resource id: 23631968, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f74c70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f74c70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115ff80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115ff80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f74c70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f74c70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 6727, resource id: 23633659, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea36a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea36a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 12386, resource id: 23634234, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c99610) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c99610) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 17921, resource id: 23634796, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e85e10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e85e10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 23500, resource id: 23635352, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1233e20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1233e20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 29100, resource id: 23635923, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12b1760) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12b1760) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 34689, resource id: 23636478, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2206340) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2206340) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 40273, resource id: 23637049, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x23ffe40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x23ffe40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 45812, resource id: 23637596, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10ccba0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10ccba0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 51376, resource id: 23638158, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x285d860) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x285d860) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x308e010) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x308e010) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1152b20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1152b20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e6e150) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e6e150) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f23f70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f23f70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e52d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e52d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e8aec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e8aec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414dd10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414dd10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f27720) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f27720) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34aac50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34aac50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e706c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e706c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1282c20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1282c20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f3fc819d570) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f3fc819d570) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414c790) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414c790) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 62437, resource id: 23639275, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e96550) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e96550) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fcaf90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fcaf90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ebf990) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ebf990) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x336bc00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x336bc00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42e27b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42e27b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f03e10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f03e10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f18010) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f18010) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d3f210) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d3f210) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f18010) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f18010) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e6af00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e6af00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35f02a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35f02a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x294e1b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x294e1b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34ead00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34ead00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12749d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12749d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 6950, resource id: 23639947, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2233a50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2233a50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 7668, resource id: 23639995, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x31a8530) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x31a8530) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ebd3f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ebd3f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1291e20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1291e20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f52d20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f52d20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34aa450) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34aa450) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4151ac0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4151ac0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
kwin_core: XCB error: 3 (BadWindow), sequence: 15354, resource id: 33554522, major code: 129 (SHAPE), minor code: 6 (Input)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34a9150) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34a9150) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
11:22:58.063 › [Notifications] notification not supported
23:10:01.206 › [Notifications] notification not supported
kwin_core: XCB error: 3 (BadWindow), sequence: 34062, resource id: 79691813, major code: 129 (SHAPE), minor code: 6 (Input)
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4150490) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4150490) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 47315, resource id: 23652270, major code: 142 (DAMAGE), minor code: 3 (Subtract)
[Parent 9747, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:9747): WARNING **: 16:39:46.481: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
kwin_core: XCB error: 3 (BadWindow), sequence: 31612, resource id: 33554546, major code: 129 (SHAPE), minor code: 6 (Input)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2ef3dd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2ef3dd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 36544, resource id: 23791365, major code: 142 (DAMAGE), minor code: 3 (Subtract)
libva info: VA-API version 1.22.0
libva info: Trying to open /usr/lib64/dri/iHD_drv_video.so
libva info: Found init function __vaDriverInit_1_22
libva info: va_openDriver() returns 0
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.private.systemtray/contents/ui/items/PlasmoidItem.qml:125: TypeError: Cannot read property 'compactRepresentationItem' of null
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
kwin_core: XCB error: 3 (BadWindow), sequence: 46280, resource id: 79691813, major code: 129 (SHAPE), minor code: 6 (Input)
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
kwin_core: XCB error: 3 (BadWindow), sequence: 10868, resource id: 33554570, major code: 129 (SHAPE), minor code: 6 (Input)
[Parent 9747, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:9747): WARNING **: 17:33:24.378: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

[Parent 9747, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:9747): WARNING **: 17:41:41.365: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
09:11:51.469 › [Notifications] notification not supported
09:16:43.105 › [Notifications] notification not supported
09:26:15.500 › [Notifications] notification not supported
09:35:46.857 › [Notifications] notification not supported
09:49:49.186 › [Notifications] notification not supported
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
kwin_core: XCB error: 3 (BadWindow), sequence: 20135, resource id: 33554589, major code: 129 (SHAPE), minor code: 6 (Input)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ebb0a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ebb0a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 26434, resource id: 23918349, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35b9030) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35b9030) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e84ff0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e84ff0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 9921, resource id: 23923452, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x358f920) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x358f920) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 14561, resource id: 23923879, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f4004115260) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f4004115260) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 24528, resource id: 23924770, major code: 142 (DAMAGE), minor code: 3 (Subtract)
12:19:53.743 › [Notifications] notification not supported
12:19:55.286 › [Notifications] notification not supported
12:20:10.174 › [Notifications] notification not supported
12:20:19.069 › [Notifications] notification not supported
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
kwin_core: XCB error: 3 (BadWindow), sequence: 49038, resource id: 33554595, major code: 129 (SHAPE), minor code: 6 (Input)
kde.dataengine.mpris: "org.mpris.MediaPlayer2.firefox.instance_1_79" does not implement org.freedesktop.DBus.Properties correctly
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.private.systemtray/contents/ui/items/PlasmoidItem.qml:125: TypeError: Cannot read property 'compactRepresentationItem' of null
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
14:40:06.824 › [Notifications] notification not supported
14:40:13.440 › [Notifications] notification not supported
14:40:18.355 › [Notifications] notification not supported
14:41:34.452 › [Notifications] notification not supported
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc6cb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc6cb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[Parent 9747, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:9747): WARNING **: 15:31:44.814: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

15:41:51.948 › [Notifications] notification not supported
15:43:50.907 › [Notifications] notification not supported
15:44:42.039 › [Notifications] notification not supported
16:10:05.594 › [Notifications] notification not supported
16:10:08.519 › [Notifications] notification not supported
16:11:56.492 › [Notifications] notification not supported
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
19:24:35.336 › [Notifications] notification not supported
21:35:28.485 › [Notifications] notification not supported
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
13:52:54.394 › [Notifications] notification not supported
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.private.systemtray/contents/ui/items/PlasmoidItem.qml:125: TypeError: Cannot read property 'compactRepresentationItem' of null
kwin_core: XCB error: 150 (BadDamage), sequence: 63410, resource id: 24052423, major code: 142 (DAMAGE), minor code: 3 (Subtract)
kf.notifications: Playing audio notification failed: Destroyed
Qt: Session management error: None of the authentication protocols specified are supported
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.taskmanager/contents/ui/Task.qml:286: Unable to assign [undefined] to QString
qt.xkb.compose: failed to create compose table
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1282200) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1282200) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 50458, resource id: 24072308, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3059cb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3059cb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 54432, resource id: 24072607, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fc0d00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fc0d00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21a7be0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21a7be0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d91c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d91c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3059cb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3059cb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34ce120) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34ce120) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34bce90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34bce90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42256c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42256c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4223680) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4223680) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e5f9d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e5f9d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f1bdb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f1bdb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 9018, resource id: 24075291, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e8fc80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e8fc80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x122b920) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x122b920) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 10165, resource id: 24075361, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9dbb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9dbb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9dbb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9dbb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea59f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea59f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34d1950) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34d1950) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e6e3c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e6e3c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41dee20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41dee20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d92010) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d92010) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3632d50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3632d50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 21118, resource id: 24076430, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f6f2d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f6f2d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e93ad0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e93ad0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41bd9d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41bd9d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414c3b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414c3b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40f4e20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40f4e20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9c480) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9c480) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fc0260) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fc0260) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 3 (BadWindow), sequence: 30428, resource id: 33554631, major code: 129 (SHAPE), minor code: 6 (Input)
LaunchProcess: failed to execvp:
xdg-open
kwin_core: XCB error: 3 (BadWindow), sequence: 51725, resource id: 62914596, major code: 129 (SHAPE), minor code: 6 (Input)
Service  ":1.83" unregistered
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f3a020) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f3a020) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 23349, resource id: 24083794, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f51ff0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f51ff0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e7690) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e7690) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f2a5a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f2a5a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33624f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33624f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40f8850) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40f8850) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3431cb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3431cb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f51ff0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f51ff0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33624f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33624f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41ad060) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41ad060) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2255350) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2255350) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x105dae0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x105dae0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 9998, resource id: 24090618, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f51ff0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f51ff0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x164f710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x164f710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x164f710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x164f710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x22327f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x22327f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3cae2d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3cae2d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x305b5c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x305b5c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f52ea0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f52ea0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3369ec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3369ec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e92ad0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e92ad0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc97e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc97e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2de49c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2de49c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4231730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4231730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12667f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12667f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ebc180) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ebc180) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ebc180) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ebc180) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x24b65e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x24b65e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x23ae580) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x23ae580) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e79de0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e79de0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f27680) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f27680) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f46cd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f46cd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f4f560) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f4f560) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f46cd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f46cd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x104a820) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x104a820) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x129fe50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x129fe50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12a64a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12a64a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f056f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f056f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed44e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed44e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1138010) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1138010) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41261b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41261b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e599b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e599b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d03e50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d03e50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e599b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e599b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115b500) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115b500) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e712e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e712e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1c9bdb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1c9bdb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e9580) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e9580) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5a230) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5a230) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e9580) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e9580) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x104a820) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x104a820) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34cab40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34cab40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1277d90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1277d90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e68b70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e68b70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3cafd50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3cafd50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f2ba20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f2ba20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3342330) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3342330) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x410d590) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x410d590) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41b7a60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41b7a60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2245120) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2245120) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f02c40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f02c40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5a230) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5a230) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x122b800) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x122b800) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x420e180) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x420e180) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5a230) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5a230) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fb3900) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fb3900) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fb3900) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fb3900) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e5b7e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e5b7e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9dbb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9dbb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41237b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41237b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3375e10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3375e10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9dbb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9dbb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x30cba80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x30cba80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 3 (BadWindow), sequence: 11591, resource id: 33554644, major code: 129 (SHAPE), minor code: 6 (Input)
[Parent 9747, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:9747): WARNING **: 11:40:09.302: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

Could not find the Plasmoid for Plasma::FrameSvgItem(0x34ddb60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34ddb60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 10453, resource id: 24105819, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f36440) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f36440) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fec580) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fec580) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41d9de0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41d9de0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12a64a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12a64a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40fd3a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40fd3a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a65e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a65e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e92780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e92780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e0d70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e0d70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x27fab60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x27fab60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42e2d80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42e2d80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x420de20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x420de20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41b65d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41b65d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41b8260) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41b8260) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fa1690) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fa1690) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4105470) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4105470) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x30b7970) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x30b7970) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fa1690) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fa1690) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2e907c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2e907c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da400) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da400) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da6c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da6c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40fbb70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40fbb70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f52840) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f52840) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f4f400) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f4f400) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f2a660) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f2a660) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a65e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a65e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3094c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3094c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f4f400) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f4f400) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x129fd30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x129fd30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x127e0f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x127e0f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x420de40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x420de40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea1bf0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea1bf0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4204000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4204000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12d5570) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12d5570) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e70b20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e70b20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1092b60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1092b60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f60880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f60880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35e96e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35e96e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e95e60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e95e60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e670b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e670b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x358e7c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x358e7c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41a41e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41a41e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc6410) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc6410) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x27faa00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x27faa00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4201b50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4201b50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4201b50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4201b50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41aced0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41aced0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10f9e80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10f9e80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10580c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10580c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f76da0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f76da0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f8f0f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f8f0f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x420d5a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x420d5a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 43220, resource id: 24126144, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34a2420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34a2420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34dd9e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34dd9e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12a64a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12a64a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12821a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12821a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f8f0f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f8f0f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9f180) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e9f180) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e8ecd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e8ecd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42e2d80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42e2d80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e9800) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e9800) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2b97c30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2b97c30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34a1eb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34a1eb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fe09d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fe09d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10987f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10987f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3faded0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3faded0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f903b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f903b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34eaca0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34eaca0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4100790) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4100790) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34cb440) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34cb440) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e84e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e84e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f7c4c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f7c4c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x410dc90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x410dc90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x305a250) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x305a250) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2245120) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2245120) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e96e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e96e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1285210) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1285210) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb0b90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb0b90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[Parent 9747, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:9747): WARNING **: 11:43:34.798: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

[Parent 9747, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:9747): WARNING **: 11:54:58.318: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
kwin_core: XCB error: 3 (BadWindow), sequence: 50323, resource id: 33554662, major code: 129 (SHAPE), minor code: 6 (Input)
kwin_core: Failed to focus 0x4a0000d (error 8)
kwin_core: XCB error: 150 (BadDamage), sequence: 9452, resource id: 24169522, major code: 142 (DAMAGE), minor code: 3 (Subtract)
kf.notifications: Playing audio notification failed: Destroyed
Qt: Session management error: None of the authentication protocols specified are supported
kwin_core: XCB error: 150 (BadDamage), sequence: 11780, resource id: 24169736, major code: 142 (DAMAGE), minor code: 3 (Subtract)
qt.xkb.compose: failed to create compose table
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
[Parent 9747, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:9747): WARNING **: 14:41:05.867: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/lib64/qml/org/kde/plasma/extras/PlaceholderMessage.qml:238:5: QML Heading: Binding loop detected for property "verticalAlignment"
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/lib64/qml/org/kde/plasma/extras/PlaceholderMessage.qml:238:5: QML Heading: Binding loop detected for property "verticalAlignment"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/contacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/emailContacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/contacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/emailContacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/contacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/emailContacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/contacts/"
org.kde.pim.akonadi_search_pim: Xapian Database does not exist at  "/afs/mpa/home/basu/.local/share/akonadi/search_db/emailContacts/"
14:43:01.356 › Logger Log level set to: info
14:43:01.445 › [App.Initialize] Current working directory is /afs/mpa/home/basu, changing into /afs/mpa/@sys/appl/mattermost-desktop-5.5.1
LaunchProcess: failed to execvp:
xdg-settings
Gtk-Message: 14:43:01.534: Failed to load module "colorreload-gtk-module"
Gtk-Message: 14:43:01.534: Failed to load module "window-decorations-gtk-module"
14:43:01.544 › [App.Config] config.autostart has been configured: true
14:43:01.553 › [App.Initialize] Autoupgrade disabled: false
14:43:01.587 › [ServerDropdownView] init
14:43:01.597 › [i18nManager] Failed to set new language en-US
14:43:01.600 › [i18nManager] Failed to set new language US
Registering ":1.123/StatusNotifierItem" to system tray
14:43:01.697 › [App.Config] config.autostart has been configured: true
14:43:02.176 › [App.Config] config.autostart has been configured: true
[9444:1104/144327.199951:ERROR:shared_image_manager.cc(217)] SharedImageManager::ProduceSkia: Trying to Produce a Skia representation from a non-existent mailbox.
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
16:35:26.972 › [Notifications] notification not supported
16:40:02.500 › [Notifications] notification not supported
16:55:36.918 › [Notifications] notification not supported
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fde640) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fde640) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3369b30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3369b30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x294e850) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x294e850) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21a8ac0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21a8ac0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x336db00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x336db00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x304dba0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x304dba0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f43900) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f43900) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21abbb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21abbb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3cb0b70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3cb0b70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x127dc20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x127dc20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
ExceptionHandler::GenerateDump attempting to generate: /afs/mpa/home/basu/.mozilla/firefox/oso3ibu6.default/minidumps/71d2ea4c-0d44-4af9-4c78-83388c18e522.dmp
ExceptionHandler::GenerateDump cloned child 3406
ExceptionHandler::SendContinueSignalToChild sent continue signal to child
ExceptionHandler::WaitForContinueSignal waiting for continue signal...
ExceptionHandler::GenerateDump minidump generation  succeeded
 Exiting due to channel error.
Exiting due to channel error.
Exiting due to channel error.
Exiting due to channel error.
Exiting due to channel error.
Exiting due to channel error.
Exiting due to channel error.
Exiting due to channel error.
Exiting due to channel error.
[GFX1-]: CompositorBridgeChild receives IPC close with reason=AbnormalShutdown
Exiting due to channel error.
Exiting due to channel error.
Exiting due to channel error.
Exiting due to channel error.
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.taskmanager/contents/ui/Task.qml:286: Unable to assign [undefined] to QString
Gtk-Message: 10:44:59.913: Failed to load module "colorreload-gtk-module"
Gtk-Message: 10:44:59.913: Failed to load module "window-decorations-gtk-module"
[Parent 3443, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:3443): WARNING **: 10:45:09.169: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d91c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d91c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 62304, resource id: 24190367, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e8ea30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e8ea30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 726, resource id: 24190671, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
kwin_core: XCB error: 3 (BadWindow), sequence: 3036, resource id: 33554680, major code: 129 (SHAPE), minor code: 6 (Input)
kwin_core: Failed to focus 0x3c0005d (error 3)
kwin_core: XCB error: 3 (BadWindow), sequence: 39255, resource id: 62914653, major code: 129 (SHAPE), minor code: 3 (Combine)
kwin_core: XCB error: 3 (BadWindow), sequence: 39256, resource id: 62914653, major code: 129 (SHAPE), minor code: 3 (Combine)
kwin_core: XCB error: 3 (BadWindow), sequence: 39277, resource id: 62914653, major code: 129 (SHAPE), minor code: 3 (Combine)
kwin_core: XCB error: 3 (BadWindow), sequence: 39278, resource id: 62914653, major code: 129 (SHAPE), minor code: 3 (Combine)
kwin_core: Failed to focus 0x3c0005f (error 3)
kwin_core: XCB error: 3 (BadWindow), sequence: 40799, resource id: 62914655, major code: 129 (SHAPE), minor code: 3 (Combine)
kwin_core: XCB error: 3 (BadWindow), sequence: 40800, resource id: 62914655, major code: 129 (SHAPE), minor code: 3 (Combine)
kwin_core: XCB error: 3 (BadWindow), sequence: 43064, resource id: 62914661, major code: 129 (SHAPE), minor code: 3 (Combine)
kwin_core: XCB error: 3 (BadWindow), sequence: 43065, resource id: 62914661, major code: 129 (SHAPE), minor code: 3 (Combine)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f75c00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f75c00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ebfc00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ebfc00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
libva info: VA-API version 1.22.0
libva info: Trying to open /usr/lib64/dri/iHD_drv_video.so
libva info: Found init function __vaDriverInit_1_22
libva info: va_openDriver() returns 0
kde.dataengine.mpris: "org.mpris.MediaPlayer2.firefox.instance_1_130" does not implement org.freedesktop.DBus.Properties correctly
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.private.systemtray/contents/ui/items/PlasmoidItem.qml:125: TypeError: Cannot read property 'compactRepresentationItem' of null
kwin_core: Failed to focus 0x3c005d9 (error 3)
kwin_core: XCB error: 3 (BadWindow), sequence: 25532, resource id: 62916057, major code: 129 (SHAPE), minor code: 3 (Combine)
kwin_core: XCB error: 3 (BadWindow), sequence: 25533, resource id: 62916057, major code: 129 (SHAPE), minor code: 3 (Combine)
kwin_core: XCB error: 3 (BadWindow), sequence: 25553, resource id: 62916057, major code: 129 (SHAPE), minor code: 3 (Combine)
kwin_core: XCB error: 3 (BadWindow), sequence: 25554, resource id: 62916057, major code: 129 (SHAPE), minor code: 3 (Combine)
kwin_core: Failed to focus 0x3c005db (error 3)
kwin_core: XCB error: 3 (BadWindow), sequence: 26795, resource id: 62916059, major code: 129 (SHAPE), minor code: 3 (Combine)
kwin_core: XCB error: 3 (BadWindow), sequence: 26796, resource id: 62916059, major code: 129 (SHAPE), minor code: 3 (Combine)
kwin_core: XCB error: 3 (BadWindow), sequence: 26820, resource id: 62916059, major code: 129 (SHAPE), minor code: 3 (Combine)
kwin_core: XCB error: 3 (BadWindow), sequence: 26821, resource id: 62916059, major code: 129 (SHAPE), minor code: 3 (Combine)
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35eb300) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35eb300) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x28606b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x28606b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
13:47:42.762 › [Notifications] notification not supported
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d308d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d308d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a4a750) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a4a750) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10d5910) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10d5910) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x272aa00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x272aa00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41abba0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41abba0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x224e640) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x224e640) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2203530) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2203530) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9ddd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9ddd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e93020) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e93020) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e1c70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e1c70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x127a470) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x127a470) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2da71b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2da71b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33e1650) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33e1650) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c6d0d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c6d0d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x105a250) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x105a250) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3364d30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3364d30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 50005, resource id: 24231687, major code: 142 (DAMAGE), minor code: 3 (Subtract)
10:32:58.295 › [Notifications] notification not supported
kwin_core: XCB error: 3 (BadWindow), sequence: 63458, resource id: 33554692, major code: 129 (SHAPE), minor code: 6 (Input)
[Parent 3443, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:3443): WARNING **: 10:41:32.177: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
11:17:10.455 › [Notifications] notification not supported
kwin_core: XCB error: 3 (BadWindow), sequence: 2409, resource id: 33554698, major code: 129 (SHAPE), minor code: 6 (Input)
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e86070) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e86070) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12b6cc0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12b6cc0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1231c70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1231c70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12c2180) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12c2180) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x225b530) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x225b530) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21ffe10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21ffe10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
17:37:45.859 › [Notifications] notification not supported
17:38:17.121 › [Notifications] notification not supported
17:38:24.389 › [Notifications] notification not supported
17:38:33.507 › [Notifications] notification not supported
17:38:41.778 › [Notifications] notification not supported
17:38:46.748 › [Notifications] notification not supported
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fe3e60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fe3e60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21ff7b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21ff7b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f11e60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f11e60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35e9240) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35e9240) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea5640) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea5640) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f67dc0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f67dc0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x27c0d90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x27c0d90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a4a750) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a4a750) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x360e060) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x360e060) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f4cb90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f4cb90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3359b90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3359b90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3091670) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3091670) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x27c07f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x27c07f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3091670) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3091670) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x285d290) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x285d290) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x285d290) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x285d290) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f940b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f940b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33d9e90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33d9e90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2241cd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2241cd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f4a2b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f4a2b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fa1ed0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fa1ed0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c65160) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c65160) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f22ff0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f22ff0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x30b1750) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x30b1750) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35b1460) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35b1460) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x305b0f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x305b0f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x121ad60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x121ad60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f4cb90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f4cb90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[Parent 3443, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:3443): WARNING **: 10:48:08.621: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4203f70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4203f70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x30cc6f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x30cc6f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
10:11:18.914 › [Notifications] notification not supported
kwin_core: XCB error: 3 (BadWindow), sequence: 11599, resource id: 33554728, major code: 129 (SHAPE), minor code: 6 (Input)
[GFX1-]: RenderCompositorSWGL failed mapping default framebuffer, no dt
kwin_core: XCB error: 3 (BadWindow), sequence: 12065, resource id: 6294770, major code: 129 (SHAPE), minor code: 6 (Input)
[Parent 3443, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:3443): WARNING **: 12:29:28.988: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
kwin_core: XCB error: 3 (BadWindow), sequence: 49312, resource id: 33554740, major code: 129 (SHAPE), minor code: 6 (Input)
kwin_core: XCB error: 150 (BadDamage), sequence: 45106, resource id: 24501837, major code: 142 (DAMAGE), minor code: 3 (Subtract)
kwin_core: XCB error: 150 (BadDamage), sequence: 45815, resource id: 24501905, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34cf3e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34cf3e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1127450) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1127450) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34cf3e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34cf3e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1127450) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1127450) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115c750) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115c750) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9860) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9860) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115c750) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115c750) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9860) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9860) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115c750) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115c750) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9860) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9860) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115c750) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115c750) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9860) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9860) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115c750) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115c750) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9860) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9860) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35f7000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35f7000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35f7000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35f7000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35f7000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35f7000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35f7000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35f7000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35f7000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35f7000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35f7000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35f7000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35f7000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35f7000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35f7000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35f7000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35f7000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35f7000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e65780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fd4c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fd4c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fd4c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fd4c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fd4c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fd4c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fd4c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fd4c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fd4c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fd4c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fd4c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fd4c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fd4c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fd4c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fb5070) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fb5070) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x22427d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x22427d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x363b2b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x363b2b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x363b2b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x363b2b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x363b2b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x363b2b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x363b2b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x363b2b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x363b2b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x363b2b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x13edcb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fb5070) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fb5070) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f27570) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f27570) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fb5070) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fb5070) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5e2c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5e2c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a2420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a2420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5e2c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5e2c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a2420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a2420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5e2c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5e2c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a2420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a2420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5e2c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5e2c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a2420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a2420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5e2c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5e2c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a2420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a2420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5e2c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5e2c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a2420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a2420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5e2c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5e2c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a2420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a2420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41f3530) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41f3530) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e8dfe0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e8dfe0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x224ccb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x224ccb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e8dfe0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e8dfe0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x224ccb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x224ccb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e8dfe0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e8dfe0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x224ccb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x224ccb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e8dfe0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e8dfe0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x224ccb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x224ccb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e8dfe0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e8dfe0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x224ccb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x224ccb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e8dfe0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e8dfe0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a2420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11a2420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5e2c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f5e2c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2de5400) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2de5400) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 52314, resource id: 24544591, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x224ccb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x224ccb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34d39b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34d39b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
10:50:39.030 › [Notifications] notification not supported
11:04:19.387 › [Notifications] notification not supported
12:20:22.695 › [Notifications] notification not supported
12:30:00.941 › [Notifications] notification not supported
14:57:41.888 › [Notifications] notification not supported
16:00:13.580 › [Notifications] notification not supported
LaunchProcess: failed to execvp:
xdg-open
LaunchProcess: failed to execvp:
xdg-open
LaunchProcess: failed to execvp:
xdg-open
LaunchProcess: failed to execvp:
xdg-open
LaunchProcess: failed to execvp:
xdg-open
LaunchProcess: failed to execvp:
xdg-open
kwin_core: XCB error: 150 (BadDamage), sequence: 39450, resource id: 24596753, major code: 142 (DAMAGE), minor code: 3 (Subtract)
[Parent 3443, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:3443): WARNING **: 17:11:14.463: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fb2f10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fb2f10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ebadd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ebadd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
13:59:08.801 › [Notifications] notification not supported
[Parent 3443, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:3443): WARNING **: 14:27:49.786: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

kwin_core: XCB error: 150 (BadDamage), sequence: 22757, resource id: 24762158, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x104ae90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x104ae90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f73e20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f73e20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x24e95c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x24e95c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x23cf9d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x23cf9d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35c83c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35c83c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9910) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9910) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1f2b1f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1f2b1f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3094f90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3094f90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10c0840) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10c0840) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3391c10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3391c10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f01570) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f01570) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c78ec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c78ec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e8bcf0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e8bcf0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x27f4330) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x27f4330) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x28af9e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x28af9e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40fb5d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40fb5d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41c8580) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41c8580) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f946e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f946e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x125e9e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x125e9e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f188d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f188d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2328900) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2328900) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x337fec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x337fec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e8ff00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e8ff00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33ad7d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33ad7d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
14:45:28.625 › [Notifications] notification not supported
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
15:57:54.366 › [Notifications] notification not supported
19:40:48.055 › [Notifications] notification not supported
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34d29d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34d29d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41ee040) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41ee040) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41b7730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41b7730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33ad7d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33ad7d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33ad7d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33ad7d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e88950) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e88950) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f43860) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f43860) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33ad7d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33ad7d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x123e2d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x123e2d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e5a740) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e5a740) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a4ab50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a4ab50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f42330) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f42330) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 3 (BadWindow), sequence: 36560, resource id: 33554782, major code: 129 (SHAPE), minor code: 6 (Input)
[Parent 3443, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:3443): WARNING **: 20:09:59.016: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

Could not find the Plasmoid for Plasma::FrameSvgItem(0x34aa240) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34aa240) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 41529, resource id: 24807632, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414c790) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414c790) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 49938, resource id: 24808476, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9a900) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9a900) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 58678, resource id: 24809439, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42e2ec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42e2ec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 63415, resource id: 24809760, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2726660) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2726660) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 34617, resource id: 24820187, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34eb140) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34eb140) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 36455, resource id: 24820485, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12325f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12325f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x122daf0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x122daf0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3377a70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3377a70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f891e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f891e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x420cc90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x420cc90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f1c8e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f1c8e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34a5230) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34a5230) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e88950) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e88950) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c6d0d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c6d0d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x420d740) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x420d740) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4151d80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4151d80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x360abc0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x360abc0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fc0b50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fc0b50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3430380) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3430380) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41aa600) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41aa600) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9150) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9150) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12b2440) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12b2440) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21ff6f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21ff6f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x22001d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x22001d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9950) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9950) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40fb5b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40fb5b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x360f570) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x360f570) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f75410) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f75410) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4130900) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4130900) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34bf3a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34bf3a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4222a70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4222a70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e64690) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e64690) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4222a70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4222a70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x422a530) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x422a530) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34df660) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34df660) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4153100) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4153100) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x125f680) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x125f680) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10c1990) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10c1990) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f06cc0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f06cc0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea3ae0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea3ae0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ebfc00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ebfc00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34df660) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34df660) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4120a00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4120a00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2391810) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2391810) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f06bf0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f06bf0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x124a220) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x124a220) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3430c40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3430c40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40f7000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40f7000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42c7080) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42c7080) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41ee0e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41ee0e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34a58e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34a58e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x422ef40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x422ef40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f1e3a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f1e3a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e91150) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e91150) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x36a8ea0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x36a8ea0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fd0040) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fd0040) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3434f70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3434f70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11381b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11381b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3434f70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3434f70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f1baa0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f1baa0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4205b40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4205b40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1982090) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1982090) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
15:40:50.093 › [Notifications] notification not supported
15:43:07.358 › [Notifications] notification not supported
00:20:53.869 › [Notifications] notification not supported
00:20:59.861 › [Notifications] notification not supported
00:21:03.047 › [Notifications] notification not supported
00:21:14.488 › [Notifications] notification not supported
00:21:28.581 › [Notifications] notification not supported
kwin_core: XCB error: 150 (BadDamage), sequence: 28752, resource id: 24795803, major code: 142 (DAMAGE), minor code: 3 (Subtract)
kwin_core: XCB error: 150 (BadDamage), sequence: 32580, resource id: 24842457, major code: 142 (DAMAGE), minor code: 3 (Subtract)
[Parent 3443, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:3443): WARNING **: 12:12:18.539: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
kwin_core: XCB error: 150 (BadDamage), sequence: 13155, resource id: 24864320, major code: 142 (DAMAGE), minor code: 3 (Subtract)
kwin_core: XCB error: 150 (BadDamage), sequence: 13973, resource id: 24864354, major code: 142 (DAMAGE), minor code: 3 (Subtract)
kwin_core: XCB error: 150 (BadDamage), sequence: 16604, resource id: 24864466, major code: 142 (DAMAGE), minor code: 3 (Subtract)
kwin_core: XCB error: 150 (BadDamage), sequence: 17748, resource id: 24864498, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
kwin_core: XCB error: 3 (BadWindow), sequence: 13325, resource id: 33554801, major code: 129 (SHAPE), minor code: 6 (Input)
Gtk-Message: 16:42:46.764: Failed to load module "colorreload-gtk-module"
Gtk-Message: 16:42:46.764: Failed to load module "window-decorations-gtk-module"
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea3ae0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea3ae0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 39731, resource id: 24901921, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f79230) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f79230) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x422cda0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x422cda0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3098030) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3098030) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f4ccc0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f4ccc0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40f5610) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40f5610) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x422cda0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x422cda0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c979d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c979d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e915d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e915d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34bd4f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34bd4f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f02e80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f02e80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x104a2a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x104a2a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4205e10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4205e10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41a9310) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41a9310) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x151a610) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x151a610) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x32f7200) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x32f7200) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x123eb60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x123eb60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42d6af0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42d6af0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e915d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e915d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x420cff0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x420cff0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f06bf0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f06bf0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10c39a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10c39a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fb2f10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fb2f10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41597f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41597f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fb41b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fb41b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f2bca0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f2bca0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x36a90a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x36a90a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f734e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f734e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eab3d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eab3d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42d7040) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42d7040) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea1360) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ea1360) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x420e160) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x420e160) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed1750) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed1750) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34bd720) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34bd720) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33624b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33624b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41efee0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41efee0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41b6630) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41b6630) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 37822, resource id: 24907904, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2ffb130) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2ffb130) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed1490) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ed1490) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2ffb130) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2ffb130) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41c9240) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41c9240) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4285a00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4285a00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x30b7970) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x30b7970) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x30b7970) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x30b7970) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x27c1540) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x27c1540) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a319e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a319e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33ad7d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33ad7d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
08:41:41.428 › [Notifications] notification not supported
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f05e70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f05e70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41c9240) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41c9240) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42127e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42127e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1285d60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1285d60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fadf00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fadf00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f0f570) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f0f570) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fadf00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fadf00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d141f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d141f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f7baf0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f7baf0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x121c950) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x121c950) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[9444:1119/111606.469254:ERROR:shared_image_manager.cc(217)] SharedImageManager::ProduceSkia: Trying to Produce a Skia representation from a non-existent mailbox.
LaunchProcess: failed to execvp:
xdg-open
LaunchProcess: failed to execvp:
xdg-open
kwin_core: XCB error: 3 (BadWindow), sequence: 35417, resource id: 65011748, major code: 129 (SHAPE), minor code: 6 (Input)
[9444:1119/112529.056743:ERROR:shared_image_manager.cc(217)] SharedImageManager::ProduceSkia: Trying to Produce a Skia representation from a non-existent mailbox.
[Parent 3443, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:3443): WARNING **: 11:39:45.097: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

[Parent 3443, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:3443): WARNING **: 11:39:54.054: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

kwin_core: XCB error: 150 (BadDamage), sequence: 63284, resource id: 24923154, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414b730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x23a50e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x23a50e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 32933, resource id: 24938208, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4207c40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4207c40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dcc000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dcc000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34b77e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34b77e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1266730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1266730) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1285ca0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1285ca0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
15:23:24.822 › [Notifications] notification not supported
15:23:32.495 › [Notifications] notification not supported
15:23:35.631 › [Notifications] notification not supported
15:23:42.429 › [Notifications] notification not supported
15:23:54.204 › [Notifications] notification not supported
15:23:56.586 › [Notifications] notification not supported
15:24:21.996 › [Notifications] notification not supported
15:24:30.736 › [Notifications] notification not supported
15:25:50.366 › [Notifications] notification not supported
15:31:53.355 › [Notifications] notification not supported
15:32:09.352 › [Notifications] notification not supported
15:32:29.625 › [Notifications] notification not supported
15:32:37.194 › [Notifications] notification not supported
15:32:59.475 › [Notifications] notification not supported
15:33:08.404 › [Notifications] notification not supported
15:33:11.236 › [Notifications] notification not supported
15:35:05.073 › [Notifications] notification not supported
15:35:33.690 › [Notifications] notification not supported
16:45:19.158 › [Notifications] notification not supported
kwin_core: XCB error: 3 (BadWindow), sequence: 44021, resource id: 33554813, major code: 129 (SHAPE), minor code: 6 (Input)
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x419b660) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x419b660) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42a51a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42a51a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb26f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eb26f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e59ee0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e59ee0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1285ab0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1285ab0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3378f10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3378f10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2ea89a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2ea89a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3caef20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3caef20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f01280) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f01280) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f89690) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f89690) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x343c720) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x343c720) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41b5cc0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41b5cc0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e714b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e714b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21a8500) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21a8500) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4157aa0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4157aa0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10cc200) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10cc200) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f439d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f439d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc74c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc74c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42309a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42309a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e6020) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e6020) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fe3d70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fe3d70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41cb940) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41cb940) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fe3d70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fe3d70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x28606b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x28606b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e4eaa0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e4eaa0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12b95c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12b95c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12b95c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12b95c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41a59e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41a59e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x360f3e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x360f3e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[9444:1120/115731.218113:ERROR:shared_image_manager.cc(217)] SharedImageManager::ProduceSkia: Trying to Produce a Skia representation from a non-existent mailbox.
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42e37c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42e37c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 17095, resource id: 24969786, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x343df20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x343df20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35b6c40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35b6c40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x32f7200) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x32f7200) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 3 (BadWindow), sequence: 9599, resource id: 33554831, major code: 129 (SHAPE), minor code: 6 (Input)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4204370) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4204370) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 17204, resource id: 24976433, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21a6440) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21a6440) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 21167, resource id: 24976731, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x343df20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x343df20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 26377, resource id: 24977075, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x32f7200) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x32f7200) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 30332, resource id: 24977371, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41a2660) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41a2660) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 34318, resource id: 24977669, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eac100) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eac100) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x121e4c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x121e4c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 10620, resource id: 24988428, major code: 142 (DAMAGE), minor code: 3 (Subtract)
kwin_core: XCB error: 150 (BadDamage), sequence: 5550, resource id: 24994392, major code: 142 (DAMAGE), minor code: 3 (Subtract)
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.taskmanager/contents/ui/Task.qml:286: Unable to assign [undefined] to QString
Qt: Session management error: None of the authentication protocols specified are supported
Qt: Session management error: None of the authentication protocols specified are supported
Cannot initialize model with data QJsonObject(). missing: QJsonValue(string, "urls")
kwin_core: XCB error: 3 (BadWindow), sequence: 11870, resource id: 79691806, major code: 129 (SHAPE), minor code: 6 (Input)
Qt: Session management error: None of the authentication protocols specified are supported
Qt: Session management error: None of the authentication protocols specified are supported
qt.xkb.compose: failed to create compose table
Could not find the Plasmoid for Plasma::FrameSvgItem(0x36aa7d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x36aa7d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 19032, resource id: 25013363, major code: 142 (DAMAGE), minor code: 3 (Subtract)
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/NotificationItem.qml:256:9: QML QQuickItem: Binding loop detected for property "height"
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/NotificationPopup.qml:106:15: QML MouseEventListener: Binding loop detected for property "height"
Qt: Session management error: None of the authentication protocols specified are supported
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41a5350) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41a5350) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 37738, resource id: 25022451, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21abb60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21abb60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
15:14:52.631 › [Notifications] notification not supported
15:14:59.796 › [Notifications] notification not supported
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
15:37:45.981 › [Notifications] notification not supported
kwin_core: XCB error: 3 (BadWindow), sequence: 6925, resource id: 33554837, major code: 129 (SHAPE), minor code: 6 (Input)
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/lib64/qml/org/kde/plasma/extras/PlaceholderMessage.qml:238:5: QML Heading: Binding loop detected for property "verticalAlignment"
kwin_core: XCB error: 150 (BadDamage), sequence: 38069, resource id: 25044169, major code: 142 (DAMAGE), minor code: 3 (Subtract)
kwin_core: XCB error: 150 (BadDamage), sequence: 39280, resource id: 25044244, major code: 142 (DAMAGE), minor code: 3 (Subtract)
kwin_core: XCB error: 150 (BadDamage), sequence: 40034, resource id: 25044273, major code: 142 (DAMAGE), minor code: 3 (Subtract)
kwin_core: XCB error: 150 (BadDamage), sequence: 45914, resource id: 25044635, major code: 142 (DAMAGE), minor code: 3 (Subtract)
[Parent 3443, Main Thread] WARNING: Attempting to store changes into '/afs/mpa/home/basu/.local/share/recently-used.xbel', but failed: Failed to create file “/afs/mpa/home/basu/.local/share/recently-used.xbel.YIUKX2”: Disk quota exceeded: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

(firefox:3443): Gtk-WARNING **: 17:04:20.058: Attempting to store changes into '/afs/mpa/home/basu/.local/share/recently-used.xbel', but failed: Failed to create file “/afs/mpa/home/basu/.local/share/recently-used.xbel.YIUKX2”: Disk quota exceeded
kf.kio.core: Failed to lock recently used
kf.kio.core: Failed to add to recently used bookmark file
kf.config.core: couldn't lock local file
Qt: Session management error: None of the authentication protocols specified are supported
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
org.kde.okular.core: Failed to open docdata file "/afs/mpa/home/basu/.local/share/okular/docdata/1227076.sigma_UV_evolution(1).pdf.xml"
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40f67c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40f67c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 47950, resource id: 25057557, major code: 142 (DAMAGE), minor code: 3 (Subtract)
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/NotificationItem.qml:256:9: QML QQuickItem: Binding loop detected for property "height"
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/NotificationPopup.qml:106:15: QML MouseEventListener: Binding loop detected for property "height"
kwin_core: XCB error: 150 (BadDamage), sequence: 53851, resource id: 25057586, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
kwin_core: XCB error: 3 (BadWindow), sequence: 12222, resource id: 33554843, major code: 129 (SHAPE), minor code: 6 (Input)
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34a0310) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34a0310) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4308510) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4308510) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eab900) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eab900) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34325c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34325c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c67680) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c67680) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34325c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34325c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[9393:1121/015504.037047:ERROR:cert_verify_proc_builtin.cc(701)] CertVerifyProcBuiltin for minervamessenger.mpdl.mpg.de failed:
----- Certificate i=0 (CN=mattermost.mpdl.mpg.de,O=Max-Planck-Gesellschaft zur F\C3\B6rderung der Wissenschaften e.V.,ST=Bayern,C=DE) -----
ERROR: Time is after notAfter


[9451:1121/015504.046542:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
[9451:1121/015603.973312:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
01:56:03.973 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/015703.973895:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
01:57:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/015803.973670:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
01:58:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/015903.974777:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
01:59:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/020003.973539:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:00:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/020103.974799:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:01:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/020203.973883:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:02:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/020303.974950:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:03:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/020403.973838:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:04:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/020503.975333:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:05:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/020603.974774:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:06:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/020703.974351:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:07:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/020803.973246:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:08:04.000 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/020903.974800:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:09:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/021003.974745:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:10:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/021103.974918:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:11:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/021203.975143:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:12:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/021303.974586:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:13:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/021403.974412:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:14:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/021503.974426:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:15:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/021603.973875:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:16:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/021703.975895:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:17:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/021803.974101:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:18:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/021903.974733:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:19:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/022003.973955:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:20:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/022103.974722:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:21:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/022203.974151:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:22:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/022303.975156:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:23:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/022403.974203:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:24:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9393:1121/022503.977767:ERROR:cert_verify_proc_builtin.cc(701)] CertVerifyProcBuiltin for minervamessenger.mpdl.mpg.de failed:
----- Certificate i=0 (CN=mattermost.mpdl.mpg.de,O=Max-Planck-Gesellschaft zur F\C3\B6rderung der Wissenschaften e.V.,ST=Bayern,C=DE) -----
ERROR: Time is after notAfter


[9451:1121/022503.978029:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:25:03.978 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/022603.974203:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:26:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/022703.974055:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:27:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/022803.973880:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:28:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/022903.974996:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:29:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/023003.975758:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:30:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/023103.975308:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:31:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/023203.974377:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:32:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/023303.974836:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:33:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/023403.974002:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:34:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/023503.975321:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:35:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/023603.974257:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:36:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/023703.976058:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:37:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/023803.975198:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:38:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/023903.976580:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:39:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/024003.975356:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:40:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/024103.976348:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:41:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1926920) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1926920) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x431c9a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x431c9a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[9451:1121/024203.975504:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:42:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/024303.976422:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:43:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/024403.974947:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:44:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/024503.976634:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:45:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/024603.978723:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:46:03.979 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/024703.976424:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:47:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/024803.975805:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:48:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/024903.976888:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:49:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/025003.975875:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:50:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/025103.975408:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:51:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/025203.977374:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:52:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/025303.975732:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:53:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/025403.979669:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:54:03.980 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
Could not find the Plasmoid for Plasma::FrameSvgItem(0x36a90d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x36a90d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x105ca70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x105ca70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[9393:1121/025503.978737:ERROR:cert_verify_proc_builtin.cc(701)] CertVerifyProcBuiltin for minervamessenger.mpdl.mpg.de failed:
----- Certificate i=0 (CN=mattermost.mpdl.mpg.de,O=Max-Planck-Gesellschaft zur F\C3\B6rderung der Wissenschaften e.V.,ST=Bayern,C=DE) -----
ERROR: Time is after notAfter


[9451:1121/025503.978982:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:55:03.979 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/025603.976590:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:56:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/025703.976191:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:57:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/025803.976630:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:58:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/025903.975484:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
02:59:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/030003.976484:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:00:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/030103.975767:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:01:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/030203.976284:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:02:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/030303.975829:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:03:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/030403.976573:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:04:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/030503.975767:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:05:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/030603.976765:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:06:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/030703.975438:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:07:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/030803.976439:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:08:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/030903.975709:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:09:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/031003.976220:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:10:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/031103.976231:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:11:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/031203.976435:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:12:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/031303.977163:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:13:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/031403.975903:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:14:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/031503.976004:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:15:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/031603.975732:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:16:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/031703.975779:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:17:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/031803.976419:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:18:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/031903.975607:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:19:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/032003.976417:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:20:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/032103.975758:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:21:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/032203.975535:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:22:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/032303.977295:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:23:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/032403.976031:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:24:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9393:1121/032503.979147:ERROR:cert_verify_proc_builtin.cc(701)] CertVerifyProcBuiltin for minervamessenger.mpdl.mpg.de failed:
----- Certificate i=0 (CN=mattermost.mpdl.mpg.de,O=Max-Planck-Gesellschaft zur F\C3\B6rderung der Wissenschaften e.V.,ST=Bayern,C=DE) -----
ERROR: Time is after notAfter


[9451:1121/032503.979439:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:25:03.979 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/032603.975772:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:26:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/032703.977663:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:27:03.978 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/032803.976050:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:28:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/032903.976576:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:29:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/033003.975430:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:30:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/033103.975820:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:31:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/033203.975220:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:32:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/033303.979616:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:33:03.980 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10639c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10639c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9a5a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9a5a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[9451:1121/033403.975505:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:34:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/033503.976466:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:35:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/033603.975685:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:36:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/033703.977468:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:37:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/033803.975716:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:38:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/033904.001045:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:39:04.001 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/034003.975727:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:40:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/034103.976394:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:41:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/034203.975262:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:42:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/034303.977046:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:43:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/034403.976234:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:44:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/034503.976122:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:45:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/034603.975649:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:46:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/034703.976343:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:47:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/034803.975570:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:48:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/034903.976102:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:49:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/035003.975511:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:50:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
Could not find the Plasmoid for Plasma::FrameSvgItem(0x43f36f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x43f36f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9a5a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3c9a5a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[9451:1121/035103.975998:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:51:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/035203.974959:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:52:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/035303.975921:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:53:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/035403.975901:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:54:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/035503.975784:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:55:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9393:1121/035603.979732:ERROR:cert_verify_proc_builtin.cc(701)] CertVerifyProcBuiltin for minervamessenger.mpdl.mpg.de failed:
----- Certificate i=0 (CN=mattermost.mpdl.mpg.de,O=Max-Planck-Gesellschaft zur F\C3\B6rderung der Wissenschaften e.V.,ST=Bayern,C=DE) -----
ERROR: Time is after notAfter


[9451:1121/035603.979896:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:56:03.980 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/035703.976351:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:57:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/035803.975716:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:58:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/035903.975988:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
03:59:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12395c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12395c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e8ea30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e8ea30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[9451:1121/040003.975553:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:00:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/040103.975804:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:01:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/040203.975752:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:02:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/040303.975922:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:03:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/040403.975563:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:04:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/040503.976272:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:05:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/040603.975811:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:06:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/040703.976490:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:07:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/040803.978831:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:08:03.979 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/040903.975831:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:09:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/041003.973654:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:10:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/041103.974288:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:11:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/041203.974018:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:12:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/041303.975360:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:13:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/041403.973676:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:14:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/041503.974767:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:15:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/041603.973773:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:16:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/041703.975918:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:17:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/041803.977088:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:18:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/041903.973418:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:19:03.973 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/042003.974484:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:20:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/042103.974215:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:21:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/042203.974278:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:22:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/042303.974224:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:23:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/042403.974237:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:24:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fa1910) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fa1910) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[9451:1121/042503.973865:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:25:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fd3040) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fd3040) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[9451:1121/042603.974498:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:26:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9393:1121/042703.977559:ERROR:cert_verify_proc_builtin.cc(701)] CertVerifyProcBuiltin for minervamessenger.mpdl.mpg.de failed:
----- Certificate i=0 (CN=mattermost.mpdl.mpg.de,O=Max-Planck-Gesellschaft zur F\C3\B6rderung der Wissenschaften e.V.,ST=Bayern,C=DE) -----
ERROR: Time is after notAfter


[9451:1121/042703.977774:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:27:03.978 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/042803.974078:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:28:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/042903.973546:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:29:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/043003.975030:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:30:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/043103.973828:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:31:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/043203.974277:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:32:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/043303.973910:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:33:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/043403.973951:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:34:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/043503.973130:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:35:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/043603.974298:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:36:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/043703.973597:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:37:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/043803.974755:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:38:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/043903.977457:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:39:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/044003.974696:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:40:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/044103.973779:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:41:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/044203.974354:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:42:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/044303.973480:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:43:03.973 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/044403.974252:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:44:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/044503.973982:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:45:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/044603.975359:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:46:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/044703.973730:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:47:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/044803.974181:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:48:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/044903.974049:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:49:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/045003.975064:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:50:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/045103.974116:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:51:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/045203.974898:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:52:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/045303.973991:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:53:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/045403.975078:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:54:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/045503.974325:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:55:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/045603.973808:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:56:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9393:1121/045703.977991:ERROR:cert_verify_proc_builtin.cc(701)] CertVerifyProcBuiltin for minervamessenger.mpdl.mpg.de failed:
----- Certificate i=0 (CN=mattermost.mpdl.mpg.de,O=Max-Planck-Gesellschaft zur F\C3\B6rderung der Wissenschaften e.V.,ST=Bayern,C=DE) -----
ERROR: Time is after notAfter


[9451:1121/045703.978232:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:57:03.978 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/045803.974635:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:58:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/045903.973970:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
04:59:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/050003.974995:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:00:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/050103.973622:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:01:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/050203.974199:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:02:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/050303.974132:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:03:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/050403.974899:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:04:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/050503.975611:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:05:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12b2440) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12b2440) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x428a060) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x428a060) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[9451:1121/050603.975111:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:06:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/050703.975015:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:07:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/050803.974588:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:08:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/050903.973366:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:09:03.973 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/051003.977323:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:10:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/051103.973849:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:11:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/051203.974700:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:12:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/051303.974514:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:13:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/051403.974199:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:14:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/051503.973531:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:15:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/051603.974381:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:16:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/051703.974235:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:17:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/051803.974608:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:18:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/051903.973767:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:19:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/052003.974386:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:20:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/052103.973680:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:21:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/052203.974071:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:22:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/052303.973799:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:23:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/052403.973618:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:24:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/052503.974047:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:25:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/052603.975092:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:26:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/052703.973888:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:27:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9393:1121/052803.977653:ERROR:cert_verify_proc_builtin.cc(701)] CertVerifyProcBuiltin for minervamessenger.mpdl.mpg.de failed:
----- Certificate i=0 (CN=mattermost.mpdl.mpg.de,O=Max-Planck-Gesellschaft zur F\C3\B6rderung der Wissenschaften e.V.,ST=Bayern,C=DE) -----
ERROR: Time is after notAfter


[9451:1121/052803.977944:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:28:03.978 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/052903.973726:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:29:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/053003.974882:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:30:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/053103.974997:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:31:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/053203.974578:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:32:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/053303.973325:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:33:03.973 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/053403.983215:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:34:03.983 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/053503.973803:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:35:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/053603.975955:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:36:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/053703.973931:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:37:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/053803.975433:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:38:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/053903.973959:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:39:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/054003.974835:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:40:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/054103.973653:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:41:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/054203.974472:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:42:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/054303.974066:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:43:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/054403.974649:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:44:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/054503.975607:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:45:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/054603.975613:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:46:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/054703.981162:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:47:03.981 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/054803.975502:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:48:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/054903.976178:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:49:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/055003.975870:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:50:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/055103.975787:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:51:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/055203.975312:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:52:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/055303.976062:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:53:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/055403.975501:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:54:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/055503.976674:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:55:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/055603.975447:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:56:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/055703.975991:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:57:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9393:1121/055803.978109:ERROR:cert_verify_proc_builtin.cc(701)] CertVerifyProcBuiltin for minervamessenger.mpdl.mpg.de failed:
----- Certificate i=0 (CN=mattermost.mpdl.mpg.de,O=Max-Planck-Gesellschaft zur F\C3\B6rderung der Wissenschaften e.V.,ST=Bayern,C=DE) -----
ERROR: Time is after notAfter


[9451:1121/055803.978259:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:58:03.978 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/055903.977306:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
05:59:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/060003.975640:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:00:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/060103.976054:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:01:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/060203.975578:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:02:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/060303.976345:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:03:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10cb420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10cb420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[9451:1121/060403.975436:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:04:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
Could not find the Plasmoid for Plasma::FrameSvgItem(0x428a060) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x428a060) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[9451:1121/060503.976458:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:05:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/060603.975184:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:06:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/060703.975822:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:07:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/060803.975705:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:08:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/060903.978559:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:09:03.978 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/061003.975699:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:10:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/061103.977031:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:11:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/061203.975719:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:12:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/061303.976588:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:13:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/061403.975342:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:14:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/061503.976496:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:15:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/061603.976456:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:16:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/061703.976529:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:17:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/061803.975266:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:18:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/061903.976352:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:19:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/062003.977322:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:20:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/062103.976316:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:21:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/062203.977109:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:22:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/062303.975735:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:23:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/062403.976353:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:24:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/062503.975815:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:25:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/062603.976441:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:26:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/062703.975504:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:27:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9393:1121/062803.980022:ERROR:cert_verify_proc_builtin.cc(701)] CertVerifyProcBuiltin for minervamessenger.mpdl.mpg.de failed:
----- Certificate i=0 (CN=mattermost.mpdl.mpg.de,O=Max-Planck-Gesellschaft zur F\C3\B6rderung der Wissenschaften e.V.,ST=Bayern,C=DE) -----
ERROR: Time is after notAfter


[9451:1121/062803.980268:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:28:03.980 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/062903.976213:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:29:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/063003.976481:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:30:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/063103.975639:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:31:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/063203.977200:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:32:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/063303.981853:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:33:03.982 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e3a60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e3a60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414c790) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x414c790) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[9451:1121/063403.976158:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:34:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/063503.976646:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:35:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/063603.975486:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:36:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/063703.975140:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:37:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/063803.975607:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:38:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/063903.975515:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:39:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/064003.975584:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:40:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/064103.976133:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:41:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/064203.976599:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:42:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/064303.975541:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:43:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/064403.976621:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:44:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/064503.975523:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:45:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/064603.977652:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:46:03.978 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/064703.975394:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:47:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/064803.976469:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:48:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/064903.975574:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:49:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/065003.977257:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:50:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/065103.975385:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:51:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/065203.976482:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:52:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/065303.974969:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:53:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/065403.976410:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:54:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/065503.976288:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:55:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/065603.975800:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:56:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fa1910) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fa1910) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2cc13a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2cc13a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[9451:1121/065703.975845:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:57:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9393:1121/065803.979075:ERROR:cert_verify_proc_builtin.cc(701)] CertVerifyProcBuiltin for minervamessenger.mpdl.mpg.de failed:
----- Certificate i=0 (CN=mattermost.mpdl.mpg.de,O=Max-Planck-Gesellschaft zur F\C3\B6rderung der Wissenschaften e.V.,ST=Bayern,C=DE) -----
ERROR: Time is after notAfter


[9451:1121/065803.979313:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:58:03.979 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/065903.975586:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
06:59:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/070003.975747:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:00:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/070103.994020:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:01:03.994 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/070203.976939:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:02:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/070303.975715:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:03:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/070403.976225:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:04:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/070503.975363:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:05:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/070603.976655:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:06:03.977 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/070703.975375:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:07:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/070803.976277:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:08:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/070903.976112:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:09:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/071003.976275:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:10:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/071103.975209:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:11:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/071203.978512:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:12:03.978 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/071303.975724:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:13:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/071403.976394:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:14:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/071503.975525:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:15:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/071603.976252:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:16:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/071703.976064:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:17:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/071803.976214:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:18:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/071903.974346:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:19:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/072003.973766:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:20:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/072103.973972:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:21:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/072203.974509:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:22:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/072303.973968:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:23:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/072403.974170:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:24:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/072503.974890:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:25:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/072603.974445:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:26:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/072703.973613:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:27:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/072803.974269:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:28:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9393:1121/072903.976449:ERROR:cert_verify_proc_builtin.cc(701)] CertVerifyProcBuiltin for minervamessenger.mpdl.mpg.de failed:
----- Certificate i=0 (CN=mattermost.mpdl.mpg.de,O=Max-Planck-Gesellschaft zur F\C3\B6rderung der Wissenschaften e.V.,ST=Bayern,C=DE) -----
ERROR: Time is after notAfter


[9451:1121/072903.976668:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:29:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/073003.974793:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:30:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/073103.973618:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:31:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/073203.973787:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:32:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/073303.973672:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:33:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/073403.974206:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:34:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/073503.973788:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:35:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/073603.974625:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:36:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/073703.973275:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:37:03.973 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/073803.974060:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:38:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/073903.973578:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:39:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/074003.974282:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:40:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/074103.975083:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:41:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/074203.974545:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:42:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/074303.974707:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:43:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/074403.974204:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:44:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/074503.973789:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:45:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/074603.975723:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:46:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/074703.973530:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:47:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/074803.974676:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:48:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/074903.974348:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:49:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/075003.974598:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:50:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/075103.976437:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:51:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/075203.974416:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:52:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/075303.974692:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:53:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/075403.974080:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:54:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/075503.973246:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:55:03.973 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc7780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc7780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[9451:1121/075603.974063:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:56:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11259c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11259c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[9451:1121/075703.973482:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:57:03.973 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/075803.974482:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:58:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9393:1121/075903.979049:ERROR:cert_verify_proc_builtin.cc(701)] CertVerifyProcBuiltin for minervamessenger.mpdl.mpg.de failed:
----- Certificate i=0 (CN=mattermost.mpdl.mpg.de,O=Max-Planck-Gesellschaft zur F\C3\B6rderung der Wissenschaften e.V.,ST=Bayern,C=DE) -----
ERROR: Time is after notAfter


[9451:1121/075903.979222:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
07:59:03.979 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/080003.974777:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
08:00:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/080103.973848:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
08:01:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/080203.974221:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
08:02:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/080303.973973:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
08:03:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9393:1121/080403.974537:ERROR:cert_verify_proc_builtin.cc(701)] CertVerifyProcBuiltin for minervamessenger.mpdl.mpg.de failed:
----- Certificate i=0 (emailAddress=minervamessenger@mpdl.mpg.de,CN=minervamessenger.mpdl.mpg.de,OU=DL,O=MPDL,L=M\C3\83\C2\BCnchen,ST=Bayern,C=DE) -----
ERROR: No matching issuer found


[9451:1121/080403.974759:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
[9451:1121/080418.852898:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:04:18.853 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080419.218377:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:04:19.218 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080420.218443:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:04:20.218 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080422.381256:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:04:22.381 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080424.217862:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:04:24.218 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080425.217982:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:04:25.218 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080426.284680:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:04:26.285 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080429.217641:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:04:29.218 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080430.218186:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:04:30.218 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080430.978094:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:04:30.978 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080434.021197:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:04:34.021 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080434.216702:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:04:34.217 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080435.217763:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:04:35.218 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080437.530709:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:04:37.531 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080439.218849:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:04:39.219 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080439.258604:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:04:39.258 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080440.736399:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:04:40.736 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080444.221325:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:04:44.221 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080444.260483:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:04:44.260 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080448.221590:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:04:48.222 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080449.220924:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:04:49.221 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080503.973523:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:05:03.973 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_AUTHORITY_INVALID
[9451:1121/080603.974497:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:06:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_AUTHORITY_INVALID
[9451:1121/080703.973988:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:07:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_AUTHORITY_INVALID
[9451:1121/080754.118747:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:07:54.119 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080801.217204:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:08:01.217 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080803.219677:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:08:03.220 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/080803.973552:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:08:03.973 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_AUTHORITY_INVALID
[9451:1121/080903.974288:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:09:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_AUTHORITY_INVALID
[9451:1121/081003.973770:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:10:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_AUTHORITY_INVALID
[9451:1121/081103.974545:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:11:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_AUTHORITY_INVALID
[9451:1121/081157.163604:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:11:57.163 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/081203.975037:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:12:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_AUTHORITY_INVALID
[9451:1121/081206.218507:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:12:06.218 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/081207.217019:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:12:07.217 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/081303.974249:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:13:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_AUTHORITY_INVALID
[9451:1121/081403.974829:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:14:03.975 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_AUTHORITY_INVALID
[9451:1121/081503.973478:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:15:03.973 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_AUTHORITY_INVALID
[9451:1121/081603.974131:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -202
08:16:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_AUTHORITY_INVALID
[9451:1121/081658.853058:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
08:16:58.853 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/081703.973254:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
08:17:03.973 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/081708.217795:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
08:17:08.218 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/081710.217145:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
08:17:10.217 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/081803.973063:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
08:18:03.973 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4312c20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4312c20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34b8e80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34b8e80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[9451:1121/081903.973803:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
08:19:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/082003.973623:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
08:20:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/082103.975635:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
08:21:03.976 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/082159.279339:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
08:21:59.279 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/082203.973082:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
08:22:03.973 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/082210.217465:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
08:22:10.217 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/082212.217041:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
08:22:12.217 › [App.App] Ignoring certificate for unmatched origin wss://minervamessenger.mpdl.mpg.de, will not trust
[9451:1121/082303.973494:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
08:23:03.973 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
[9451:1121/082403.974135:ERROR:ssl_client_socket_impl.cc(968)] handshake failed; returned -1, SSL error code 1, net_error -201
08:24:03.974 › [App.App] Ignoring already shown dialog for https://minervamessenger.mpdl.mpg.de:net::ERR_CERT_DATE_INVALID
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3333660) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3333660) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x430a690) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x430a690) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21a4e30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21a4e30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40f67c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40f67c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x22001d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x22001d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x432ea10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x432ea10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11257b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x11257b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x279b100) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x279b100) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 36509, resource id: 25069948, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Service  ":1.123" unregistered
09:55:50.468 › Logger Log level set to: info
09:55:50.544 › [App.Initialize] Current working directory is /afs/mpa/home/basu, changing into /afs/mpa/@sys/appl/mattermost-desktop-5.5.1
LaunchProcess: failed to execvp:
xdg-settings
Gtk-Message: 09:55:50.576: Failed to load module "colorreload-gtk-module"
Gtk-Message: 09:55:50.576: Failed to load module "window-decorations-gtk-module"
09:55:50.588 › [App.Config] config.autostart has been configured: true
09:55:50.597 › [App.Initialize] Autoupgrade disabled: false
09:55:50.624 › [ServerDropdownView] init
09:55:50.634 › [i18nManager] Failed to set new language en-US
09:55:50.637 › [i18nManager] Failed to set new language US
Registering ":1.174/StatusNotifierItem" to system tray
09:55:50.660 › [App.Config] config.autostart has been configured: true
09:55:51.102 › [App.Config] config.autostart has been configured: true
[940:1121/095707.982335:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1121/095928.387126:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[940:1121/100043.337137:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1121/100434.217412:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1121/100828.355016:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
Could not find the Plasmoid for Plasma::FrameSvgItem(0x223a710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x223a710) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 42618, resource id: 25077337, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41aaec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41aaec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[940:1121/102231.377464:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1121/102349.787170:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1121/102459.316677:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1121/103035.717617:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[940:1121/103528.377051:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1121/103831.327296:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1121/104930.357152:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
[940:1121/105547.307282:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1121/105813.217208:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1121/110125.217229:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21af4c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21af4c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x419b3c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x419b3c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[940:1121/110355.222563:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1121/111425.216657:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1121/111725.222753:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1121/111955.227207:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1121/112237.327389:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1121/112425.227478:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1121/112925.217163:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1121/113425.221979:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[940:1121/113828.218220:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
LaunchProcess: failed to execvp:
xdg-open
kwin_core: XCB error: 3 (BadWindow), sequence: 10633, resource id: 65011743, major code: 129 (SHAPE), minor code: 6 (Input)
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[940:1121/114352.456886:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[940:1121/115945.727307:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[940:1121/123532.037304:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10d4490) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10d4490) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x36a77b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x36a77b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115d170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115d170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 34198, resource id: 25102016, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x36a77b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x36a77b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 38777, resource id: 25102314, major code: 142 (DAMAGE), minor code: 3 (Subtract)
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f44360) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f44360) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4279bb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4279bb0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x347d510) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x347d510) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x43f27e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x43f27e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e54890) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e54890) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4234100) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4234100) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x15fcc20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x15fcc20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x430a4d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x430a4d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41c97b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41c97b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x419c670) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x419c670) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 57602, resource id: 25104902, major code: 142 (DAMAGE), minor code: 3 (Subtract)
kwin_core: XCB error: 3 (BadWindow), sequence: 59005, resource id: 81788962, major code: 129 (SHAPE), minor code: 6 (Input)
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'pageload#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'pageload#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40fb210) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x40fb210) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x430a4d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x430a4d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41c97b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41c97b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x347d550) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x347d550) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
Could not find the Plasmoid for Plasma::FrameSvgItem(0x352aec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x352aec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 11547, resource id: 25112865, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42832f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42832f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 17738, resource id: 25113318, major code: 142 (DAMAGE), minor code: 3 (Subtract)
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[Parent 3443, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:3443): WARNING **: 20:21:23.722: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[Parent 3443, Unnamed thread 7f747b685160] WARNING: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.1WSJX2”: Disk quota exceeded: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

(firefox:3443): dconf-WARNING **: 20:33:31.108: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.1WSJX2”: Disk quota exceeded
[Parent 3443, Main Thread] WARNING: Attempting to store changes into '/afs/mpa/home/basu/.local/share/recently-used.xbel', but failed: Failed to create file “/afs/mpa/home/basu/.local/share/recently-used.xbel.E0TJX2”: Disk quota exceeded: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

(firefox:3443): Gtk-WARNING **: 20:33:31.113: Attempting to store changes into '/afs/mpa/home/basu/.local/share/recently-used.xbel', but failed: Failed to create file “/afs/mpa/home/basu/.local/share/recently-used.xbel.E0TJX2”: Disk quota exceeded
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[Parent 3443, Unnamed thread 7f747b685160] WARNING: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.XLA5W2”: Disk quota exceeded: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

(firefox:3443): dconf-WARNING **: 20:33:44.808: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.XLA5W2”: Disk quota exceeded
[ERROR glean_core::database] Failed to record metric 'events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
"Could not write to file /afs/mpa/home/basu/.local/share/Trash/info/deltaTB.png.trashinfo."
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
kwin_core: XCB error: 150 (BadDamage), sequence: 57853, resource id: 25137227, major code: 142 (DAMAGE), minor code: 3 (Subtract)
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21ddff0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21ddff0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 33528, resource id: 23438835, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4213850) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4213850) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 59601, resource id: 25142970, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3526e40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3526e40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4208f10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4208f10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f4c910) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f4c910) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 7802, resource id: 23453172, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2b80ad0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2b80ad0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a38260) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a38260) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 20286, resource id: 23454008, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x334ea10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x334ea10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x334ea10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x334ea10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x350d8d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x350d8d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x334ea10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x334ea10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 37430, resource id: 23455564, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x334ea10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x334ea10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a2bdd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a2bdd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a2bdd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a2bdd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x25631c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x25631c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a2bdd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a2bdd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x43f2d90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x43f2d90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4103660) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4103660) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42e2ec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42e2ec0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x27beb80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x27beb80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2cee8d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2cee8d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41ab290) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41ab290) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fc1d20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fc1d20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35c8870) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35c8870) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 10668, resource id: 23459152, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x309f610) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x309f610) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x308b9b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x308b9b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 17106, resource id: 24843291, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
LaunchProcess: failed to execvp:
xdg-open
LaunchProcess: failed to execvp:
xdg-open
kwin_core: XCB error: 3 (BadWindow), sequence: 53968, resource id: 65011749, major code: 129 (SHAPE), minor code: 6 (Input)
LaunchProcess: failed to execvp:
xdg-open
kwin_core: XCB error: 3 (BadWindow), sequence: 54657, resource id: 65011750, major code: 129 (SHAPE), minor code: 6 (Input)
[935:1122/171235.021102:ERROR:shared_image_manager.cc(217)] SharedImageManager::ProduceSkia: Trying to Produce a Skia representation from a non-existent mailbox.
[Parent 3443, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:3443): WARNING **: 17:29:07.441: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

[Parent 3443, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:3443): WARNING **: 17:45:39.209: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
[935:1122/185357.094868:ERROR:gl_surface_presentation_helper.cc(260)] GetVSyncParametersIfAvailable() failed for 1 times!
[935:1122/191602.449653:ERROR:gl_surface_presentation_helper.cc(260)] GetVSyncParametersIfAvailable() failed for 2 times!
[Parent 3443, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:3443): WARNING **: 19:32:39.381: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e5e090) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e5e090) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x30503e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x30503e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21d0e70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21d0e70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34ec860) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34ec860) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x43da420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x43da420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12b6620) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12b6620) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10d4490) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10d4490) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x361fd00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x361fd00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4284000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4284000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3611540) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3611540) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1131c90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1131c90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3611540) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3611540) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x31d00c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x31d00c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34dd740) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34dd740) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115d170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115d170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 64191, resource id: 23857554, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3386720) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3386720) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eaaa20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eaaa20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21a6c40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21a6c40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2bd3a50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2bd3a50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x339c9b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x339c9b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e5fa30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e5fa30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x339c9b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x339c9b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34b7680) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34b7680) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x27beb80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x27beb80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x36ac220) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x36ac220) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f33390) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f33390) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3503fd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3503fd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3503fd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3503fd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x36ac220) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x36ac220) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f691d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f691d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12c47d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12c47d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3392720) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3392720) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41ab290) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41ab290) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12c47d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12c47d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fc1d20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fc1d20) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12b6620) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12b6620) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12222e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12222e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33532a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x33532a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
15:36:08.640 › [Notifications] notification not supported
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1f2f720) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1f2f720) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da950) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41da950) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 106, resource id: 23947140, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x305cbe0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x305cbe0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x36ac220) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x36ac220) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x124b180) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x124b180) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x36ac220) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x36ac220) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115d170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x115d170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42040c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42040c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x43da420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x43da420) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34dd740) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34dd740) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x43e5050) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x43e5050) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2bb0d70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2bb0d70) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f44a60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f44a60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f3d2d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f3d2d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f42930) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f42930) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f09090) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f09090) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4103660) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4103660) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4225ca0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4225ca0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41c1790) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41c1790) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4441510) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4441510) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41c1790) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41c1790) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a3a1a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a3a1a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1246c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1246c80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3364780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3364780) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
08:53:30.483 › [Notifications] notification not supported
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f40c30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f40c30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e3a60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e3a60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10fc1f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x10fc1f0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e3a60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34e3a60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x126e200) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x126e200) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2b64060) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2b64060) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3611540) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3611540) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42e92e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x42e92e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 3 (BadWindow), sequence: 40580, resource id: 33554904, major code: 129 (SHAPE), minor code: 6 (Input)
kwin_core: XCB error: 150 (BadDamage), sequence: 49971, resource id: 24047006, major code: 142 (DAMAGE), minor code: 3 (Subtract)
kwin_core: XCB error: 150 (BadDamage), sequence: 51762, resource id: 24047117, major code: 142 (DAMAGE), minor code: 3 (Subtract)
kf.notifications: Playing audio notification failed: Destroyed
kwin_core: XCB error: 150 (BadDamage), sequence: 52955, resource id: 23693544, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
kwin_core: XCB error: 3 (BadWindow), sequence: 3410, resource id: 33554910, major code: 129 (SHAPE), minor code: 6 (Input)
[Parent 3443, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:3443): WARNING **: 12:12:39.134: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files


malloc: unknown:0: assertion botched
free: start and end chunk sizes differ
Aborting...Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.taskmanager/contents/ui/Task.qml:286: Unable to assign [undefined] to QString
Qt: Session management error: None of the authentication protocols specified are supported
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
08:45:48.189 › [Notifications] notification not supported
qt.xkb.compose: failed to create compose table
kwin_core: XCB error: 3 (BadWindow), sequence: 37113, resource id: 65011751, major code: 129 (SHAPE), minor code: 6 (Input)
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
[935:1127/005953.499703:ERROR:gl_surface_presentation_helper.cc(260)] GetVSyncParametersIfAvailable() failed for 3 times!
08:15:51.980 › [Notifications] notification not supported
kwin_core: XCB error: 3 (BadWindow), sequence: 60259, resource id: 79691810, major code: 129 (SHAPE), minor code: 6 (Input)
[Parent 3443, IPC I/O Parent] WARNING: process 14956 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
LaunchProcess: failed to execvp:
xdg-open
[935:1127/112718.175627:ERROR:shared_image_manager.cc(217)] SharedImageManager::ProduceSkia: Trying to Produce a Skia representation from a non-existent mailbox.
LaunchProcess: failed to execvp:
xdg-open
kwin_core: XCB error: 3 (BadWindow), sequence: 4394, resource id: 65011754, major code: 129 (SHAPE), minor code: 6 (Input)
[Parent 3443, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:187

** (firefox:3443): WARNING **: 11:27:26.488: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

[Parent 3443, IPC I/O Parent] WARNING: process 15140 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15142 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15145 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15148 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15150 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15152 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15154 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15156 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15158 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15160 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15162 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15164 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15166 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15168 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15170 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15172 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15174 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15176 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15178 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15180 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15182 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15184 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15186 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15188 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15190 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15192 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15194 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15196 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15198 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15200 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15202 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15204 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15206 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15208 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15210 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15212 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15214 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15216 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15218 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15220 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15222 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15224 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15226 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15228 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15230 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15232 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15234 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15236 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15238 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15240 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15242 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15244 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15246 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15248 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15250 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15252 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15254 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15256 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15258 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15260 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15262 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15264 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15266 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15268 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15270 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15272 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15274 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15276 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15278 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15280 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15282 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15284 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15286 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15288 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15290 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15292 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15294 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15296 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15298 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15300 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15302 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15304 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15306 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15308 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15310 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15312 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15314 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15316 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15318 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15320 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15322 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15324 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15326 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15328 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15330 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15332 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15334 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15336 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15338 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15340 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15342 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15344 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15346 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15348 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15350 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15352 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15354 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15356 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15358 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15360 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15362 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15364 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15366 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15368 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15370 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15372 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15374 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15376 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15378 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15380 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15382 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15384 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15386 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15388 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15390 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15392 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15394 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15396 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15398 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15400 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15402 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15404 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15406 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15408 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15410 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15412 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15414 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15416 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15418 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15420 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15422 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15424 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15426 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15428 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15430 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15432 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15434 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15436 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15438 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15440 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15442 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15444 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15446 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15448 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15450 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15452 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15454 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15456 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15458 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15460 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15462 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15464 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15466 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15468 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15470 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15472 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15474 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15476 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15478 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15480 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15482 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15484 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15486 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15488 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15490 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15492 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15494 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15496 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15498 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15500 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15502 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15504 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15506 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15508 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15510 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15512 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15514 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15516 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15518 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15520 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15522 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15524 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15526 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15528 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15530 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15532 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15534 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15536 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15538 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15540 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15542 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15544 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15546 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15548 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15550 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15552 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15554 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15556 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15558 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15560 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15562 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15564 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15566 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15568 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15570 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15572 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15574 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15576 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15578 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15580 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15582 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15584 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15586 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15588 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15590 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15592 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15594 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15596 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15598 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15600 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15602 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15604 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15606 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15608 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15610 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15612 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15614 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15616 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15618 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15620 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15622 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15624 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15626 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15628 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15630 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15632 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15634 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15636 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15638 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15640 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15642 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15644 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15646 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15648 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15650 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15652 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15654 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15656 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15658 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15660 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15662 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15664 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15666 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15668 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15670 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15672 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15674 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15676 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15678 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15680 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15682 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15684 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15686 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15688 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15690 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15692 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15694 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15696 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15698 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15700 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15702 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15704 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15706 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15708 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15710 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15712 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15714 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15716 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15718 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15720 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15722 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15724 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15726 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15728 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15730 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15732 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15734 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15736 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15738 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15740 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15742 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15744 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15746 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15748 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15750 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15752 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15754 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15756 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15758 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15760 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15762 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15764 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15766 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15768 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15770 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15772 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15774 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15776 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15778 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15780 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15782 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15784 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15786 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15788 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15790 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15792 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15794 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15796 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15798 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15800 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15802 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15804 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15806 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15808 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15810 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15812 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15814 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15816 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15818 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15820 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15822 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15824 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15826 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15828 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15830 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15832 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15834 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15836 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15838 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15840 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15842 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15844 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15846 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15848 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15850 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15852 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15854 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15856 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15858 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15860 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15862 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15864 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15866 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15868 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15870 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15872 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15874 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15876 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15878 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15880 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15882 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15884 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15886 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15888 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15890 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15892 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15894 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15896 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15898 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15900 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15902 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15904 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15906 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15908 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15910 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15912 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15914 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15916 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15918 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15920 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15922 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15924 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15926 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15928 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15930 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15932 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15934 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15936 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15938 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15940 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15942 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15944 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15946 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15948 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15950 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15952 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15954 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15956 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15958 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15960 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15962 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15964 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15966 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15968 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15970 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15972 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15974 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15976 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15978 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15980 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15982 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15984 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15986 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15988 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15990 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15992 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15994 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15996 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 15998 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16000 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16002 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16004 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16006 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16008 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16010 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16012 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16014 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16016 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16018 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16020 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16022 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16024 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16026 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16028 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16030 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16032 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16034 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16036 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16038 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16040 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16042 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16044 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16046 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16048 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16050 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16052 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16054 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16056 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16058 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16060 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16062 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16064 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16066 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16068 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16070 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16072 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16074 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16076 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16078 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16080 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16082 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16084 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16086 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16088 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16090 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16092 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16094 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16096 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16098 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16100 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16102 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16104 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16106 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16108 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16110 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16112 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16114 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16116 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16118 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16120 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16122 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16124 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16126 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16128 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16130 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16132 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16134 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16136 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16138 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16140 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16142 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16144 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16146 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16148 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16150 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16152 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16154 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16156 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16158 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16160 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16162 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16164 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16166 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16168 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16170 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16172 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16174 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16176 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16178 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16180 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16182 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16184 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16186 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16188 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16190 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16192 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16194 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16196 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16198 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16200 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16202 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16204 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16206 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16208 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16210 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16212 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16214 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16216 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16218 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16220 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16222 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16224 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16226 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16228 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16394 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16396 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16398 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16400 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16402 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16404 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16406 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16408 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16410 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16413 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16415 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16417 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16419 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16421 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16423 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16425 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16427 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16429 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16431 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16433 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16435 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16437 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16439 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16441 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16443 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16445 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16447 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16449 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16451 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16453 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16455 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16457 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16459 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16461 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16463 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16465 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16467 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16469 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16471 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16473 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16475 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16477 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16479 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16481 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16483 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16485 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16487 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16489 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16491 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16493 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16495 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16497 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16499 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16501 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16503 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16505 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16507 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16509 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16511 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16513 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16515 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16517 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16519 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16521 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16523 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16525 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16527 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16529 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16531 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16533 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16535 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16537 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16539 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16541 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16543 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16545 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16547 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16549 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16552 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16554 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16556 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16558 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16560 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16562 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16564 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16566 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16568 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16570 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16572 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16574 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16576 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16578 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16580 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16582 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16584 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16586 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16588 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16590 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16592 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16594 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16596 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16598 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16600 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16602 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16604 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16606 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16608 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16610 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[ERROR buildid_reader::reader] BuildIdReader::new failed to open "/afs/mpa/@sys/appl/firefox/firefox-132.0/libxul.so" with error No such file or directory (os error 2)
[ERROR buildid_reader] read_toolkit_buildid_from_file failed to build BuildIdReader for "/afs/mpa/@sys/appl/firefox/firefox-132.0/libxul.so" with error NS_ERROR_ILLEGAL_VALUE
[Parent 3443, IPC I/O Parent] WARNING: process 16876 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[ERROR buildid_reader::reader] BuildIdReader::new failed to open "/afs/mpa/@sys/appl/firefox/firefox-132.0/libxul.so" with error No such file or directory (os error 2)
[ERROR buildid_reader] read_toolkit_buildid_from_file failed to build BuildIdReader for "/afs/mpa/@sys/appl/firefox/firefox-132.0/libxul.so" with error NS_ERROR_ILLEGAL_VALUE
[Parent 3443, IPC I/O Parent] WARNING: process 16881 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16895 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16897 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16899 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16901 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16903 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16906 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16908 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16910 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16912 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16914 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16916 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16918 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16920 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16922 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16924 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16926 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16928 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16930 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16932 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16934 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16936 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16938 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16940 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16942 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16944 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16946 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16948 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16950 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16952 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16954 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16956 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16958 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16960 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16962 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16964 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16966 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16968 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16970 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16972 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16974 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16976 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16978 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16980 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16982 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16984 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16986 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16988 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16990 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16992 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16994 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16996 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 16998 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17000 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17002 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17004 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17006 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17008 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17010 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17012 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17014 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17016 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17018 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17020 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17022 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17024 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17026 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17028 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17030 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17032 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17034 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17036 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17038 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17040 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17042 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17044 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17046 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17048 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17050 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17052 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[ERROR buildid_reader::reader] BuildIdReader::new failed to open "/afs/mpa/@sys/appl/firefox/firefox-132.0/libxul.so" with error No such file or directory (os error 2)
[ERROR buildid_reader] read_toolkit_buildid_from_file failed to build BuildIdReader for "/afs/mpa/@sys/appl/firefox/firefox-132.0/libxul.so" with error NS_ERROR_ILLEGAL_VALUE
[Parent 3443, IPC I/O Parent] WARNING: process 17054 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17056 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17058 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17060 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17062 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17064 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17066 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17068 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17070 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17072 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17074 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17076 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17078 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17080 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17082 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17084 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17086 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17088 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17090 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17092 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17094 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17096 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17098 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17101 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17103 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17105 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17107 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17109 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17111 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17113 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17115 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17117 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17119 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17121 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17123 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17125 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17127 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17129 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17131 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17133 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17135 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17137 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17139 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17141 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17143 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17145 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17147 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17149 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17151 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17153 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17155 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17157 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17159 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17161 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17163 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17165 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17167 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17169 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17171 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17173 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17175 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17177 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17179 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17181 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17183 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17185 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17187 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17189 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17191 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17193 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17195 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17197 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17199 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17201 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17203 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17205 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17207 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17209 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17211 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17213 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17215 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17217 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17219 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17221 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17223 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17225 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17227 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17229 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17231 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17233 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17235 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17237 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17239 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17241 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17243 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17245 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17247 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17249 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17251 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17253 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17255 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17257 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17259 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17261 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17263 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17265 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17267 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17269 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17271 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17273 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17275 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17277 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17279 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17281 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17283 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17285 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17287 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17289 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17291 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17293 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17295 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17297 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17299 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17301 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17303 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17305 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17307 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17309 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17311 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17313 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17315 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17317 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17319 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17321 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17323 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17325 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17327 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17329 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17331 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17333 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17335 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17337 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17339 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17341 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17343 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17345 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17347 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17349 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17351 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17353 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17355 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17357 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17359 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17361 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17363 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17365 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17367 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17369 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17371 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17373 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17375 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17377 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17379 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17381 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17383 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17385 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17387 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17389 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17391 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17393 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17395 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17397 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17399 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17401 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17403 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17405 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17407 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17409 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17411 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17413 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17415 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17417 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17419 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17421 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17423 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17425 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17427 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17429 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17431 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17433 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17435 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17437 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17439 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17441 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17443 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17445 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17447 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17449 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17451 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17453 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17455 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17457 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17459 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17461 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17463 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17465 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17467 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17469 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17471 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17473 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17475 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17477 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17479 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17481 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17483 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17485 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17487 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17489 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17491 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17493 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17495 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17497 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17499 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17501 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17503 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17505 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17507 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17509 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17511 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17513 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17515 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17517 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17519 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17521 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17523 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17525 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17527 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17529 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17531 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17533 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17535 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17537 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17539 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17541 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17543 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
kwin_core: XCB error: 150 (BadDamage), sequence: 5422, resource id: 24189637, major code: 142 (DAMAGE), minor code: 3 (Subtract)
[Parent 3443, IPC I/O Parent] WARNING: process 17545 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
[Parent 3443, IPC I/O Parent] WARNING: process 17547 exited with status 127: file /builds/worker/checkouts/gecko/ipc/chromium/src/base/process_util_posix.cc:341
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.taskmanager/contents/ui/Task.qml:286: Unable to assign [undefined] to QString
Gtk-Message: 11:49:35.880: Failed to load module "colorreload-gtk-module"
Gtk-Message: 11:49:35.880: Failed to load module "window-decorations-gtk-module"
[Parent 17581, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:201

** (firefox:17581): WARNING **: 11:49:51.849: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

[Parent 17581, Main Thread] WARNING: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files
: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:201

** (firefox:17581): WARNING **: 12:21:29.519: Failed to enumerate devices of org.freedesktop.UPower: GDBus.Error:org.freedesktop.DBus.Error.ServiceUnknown: The name org.freedesktop.UPower was not provided by any .service files

Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
14:00:37.999 › [Notifications] notification not supported
Could not find the Plasmoid for Plasma::FrameSvgItem(0x371e3b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x371e3b0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1091b50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1091b50) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x336c5d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x336c5d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f19e10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f19e10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x22081c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x22081c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4107120) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4107120) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3611540) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3611540) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2234e80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2234e80) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 150 (BadDamage), sequence: 47768, resource id: 23937208, major code: 142 (DAMAGE), minor code: 3 (Subtract)
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34eb180) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34eb180) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4107120) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4107120) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2c5ec60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2c5ec60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4107120) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4107120) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41eb6d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x41eb6d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e50510) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1e50510) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x43e5050) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x43e5050) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x43e5050) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x43e5050) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3502850) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3502850) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f33140) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2f33140) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0xe2fe60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0xe2fe60) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x430c580) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x430c580) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35b6c40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35b6c40) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f19e10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f19e10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12411a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x12411a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fb5030) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3fb5030) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x440e3a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x440e3a0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x122c320) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x122c320) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34b7680) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34b7680) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
kwin_core: XCB error: 3 (BadWindow), sequence: 34416, resource id: 33554956, major code: 129 (SHAPE), minor code: 6 (Input)
kwin_core: Failed to focus 0x3c0000d (error 8)
kwin_core: Failed to focus 0x3c0000d (error 8)
kwin_core: XCB error: 150 (BadDamage), sequence: 48034, resource id: 23944884, major code: 142 (DAMAGE), minor code: 3 (Subtract)
kf.notifications: Playing audio notification failed: Destroyed
Qt: Session management error: None of the authentication protocols specified are supported
qt.xkb.compose: failed to create compose table
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21ddff0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21ddff0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34dd740) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34dd740) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3585000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3585000) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2b04010) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2b04010) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21e5680) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x21e5680) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34dd740) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x34dd740) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x45b3ad0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x45b3ad0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2b04010) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2b04010) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x45b3ad0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x45b3ad0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fd1400) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2fd1400) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
kwin_core: XCB error: 3 (BadWindow), sequence: 11539, resource id: 33554962, major code: 129 (SHAPE), minor code: 6 (Input)
[GFX1-]: RenderCompositorSWGL failed mapping default framebuffer, no dt
kwin_core: XCB error: 150 (BadDamage), sequence: 39178, resource id: 23910772, major code: 142 (DAMAGE), minor code: 3 (Subtract)
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.taskmanager/contents/ui/Task.qml:286: Unable to assign [undefined] to QString
Gtk-Message: 16:56:34.837: Failed to load module "colorreload-gtk-module"
Gtk-Message: 16:56:34.837: Failed to load module "window-decorations-gtk-module"
kwin_core: XCB error: 150 (BadDamage), sequence: 42297, resource id: 23951512, major code: 142 (DAMAGE), minor code: 3 (Subtract)
[15181] Sandbox: Unexpected EOF, op 0 flags 00 path /proc/cpuinfo
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f09090) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f09090) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a416d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2a416d0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
17:37:39.281 › [Notifications] notification not supported
17:39:45.557 › [Notifications] notification not supported
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35eec30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35eec30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e91790) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e91790) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
19:10:01.109 › [Notifications] notification not supported
19:14:53.511 › [Notifications] notification not supported
19:15:09.069 › [Notifications] notification not supported
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35eec30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35eec30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e91790) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3e91790) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35eec30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x35eec30) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4310e10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4310e10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb7170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb7170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
20:20:11.777 › [Notifications] notification not supported
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb7170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb7170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
20:48:33.899 › [Notifications] notification not supported
20:49:00.606 › [Notifications] notification not supported
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb7170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb7170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb7170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb7170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb7170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb7170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb7170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb7170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb7170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb7170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb7170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb7170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb7170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb7170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb7170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eb7170) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3eff880) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.taskmanager/contents/ui/Task.qml:286: Unable to assign [undefined] to QString
Gtk-Message: 11:26:43.694: Failed to load module "colorreload-gtk-module"
Gtk-Message: 11:26:43.695: Failed to load module "window-decorations-gtk-module"
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/lib64/qml/org/kde/plasma/extras/PlaceholderMessage.qml:238:5: QML Heading: Binding loop detected for property "verticalAlignment"
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/lib64/qml/org/kde/plasma/extras/PlaceholderMessage.qml:238:5: QML Heading: Binding loop detected for property "verticalAlignment"
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/lib64/qml/org/kde/plasma/extras/PlaceholderMessage.qml:238:5: QML Heading: Binding loop detected for property "verticalAlignment"
libva info: VA-API version 1.22.0
libva info: Trying to open /usr/lib64/dri/iHD_drv_video.so
libva info: Found init function __vaDriverInit_1_22
libva info: va_openDriver() returns 0
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f4144048800) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f4144048800) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f09090) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3f09090) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f414403dbd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x7f414403dbd0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x22362c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x22362c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3611540) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3611540) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ca0630) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3ca0630) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1131c90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x1131c90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d833e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d833e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x408b910) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x408b910) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2deff10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2deff10) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9920) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3dc9920) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x352f280) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x352f280) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4418d00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x4418d00) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x335b590) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x335b590) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eabb90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2eabb90) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[940:1201/161031.337730:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1201/162331.807287:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1201/164628.327315:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1201/170443.797436:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1201/172128.337282:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1201/174301.287089:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1201/180646.327144:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1201/183128.847167:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1201/192549.784975:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1201/200328.867607:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1201/210249.297276:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1201/213131.286929:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1201/214046.324807:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1201/214528.837218:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1201/215852.307599:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1201/221631.807157:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1201/222034.202598:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1201/222058.782233:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1201/222431.365776:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1201/225152.296944:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1201/232140.297349:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1201/233928.847295:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/001131.297806:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d833e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d833e0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3575690) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x3575690) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[940:1202/002246.303149:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/002528.807376:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/004237.337422:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/004628.727121:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/011855.287333:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2ae51c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2ae51c0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d5cbe0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
Could not find the Plasmoid for Plasma::FrameSvgItem(0x2d5cbe0) QQmlContext(0x25060c0) QUrl("file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.notifications/contents/ui/global/Globals.qml")
[940:1202/012937.297152:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/013228.857270:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/013652.296718:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/014231.357452:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/020355.797181:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/023729.227001:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/024501.276966:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/025440.297166:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/031331.297172:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/031534.807475:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/034028.337139:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/035658.297200:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[ERROR glean_core::database] Failed to record metric 'metrics#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'metrics#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'mps.last_sent_time' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[940:1202/040331.297268:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/041631.287417:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/043228.337127:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/043531.797181:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/051149.297172:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/055828.220374:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/060625.217318:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/060831.316241:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/061022.216941:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/062340.237251:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/065725.217272:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/072225.223165:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/075925.225653:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/082107.227250:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/082825.225188:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/083925.221574:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/084625.227280:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/090355.227234:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/090928.226504:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/091155.227396:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/094828.223206:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/095852.257028:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/100322.226962:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/101022.227606:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/101531.827150:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/104128.354897:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/104734.203947:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/104825.223414:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/105325.217509:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/105943.227143:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/110410.217223:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/110925.223212:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/112125.217229:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/112655.237506:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/113128.227121:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'pageload#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'pageload#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[940:1202/115522.222744:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[881:1202/120341.737270:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/120344.776931:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
kwin_core: Failed to focus 0x3c0000d (error 8)
kwin_core: Failed to focus 0x3c0000d (error 8)
kwin_core: XCB error: 150 (BadDamage), sequence: 30374, resource id: 24379411, major code: 142 (DAMAGE), minor code: 3 (Subtract)
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
file:///afs/mpa/@sys/appl/kde-5.27.11_14.23/share/plasma/plasmoids/org.kde.plasma.taskmanager/contents/ui/Task.qml:286: Unable to assign [undefined] to QString
Qt: Session management error: None of the authentication protocols specified are supported
kf.config.core: couldn't lock local file
kf.config.core: couldn't lock local file
qt.xkb.compose: failed to create compose table
[940:1202/120537.204789:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[940:1202/120616.217296:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[GFX1-]: RenderCompositorSWGL failed mapping default framebuffer, no dt
[940:1202/120840.226778:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[940:1202/123031.202122:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/123107.217411:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
Qt: Session management error: networkIdsList argument is NULL
virtual QStringList Solid::Backends::UPower::UPowerManager::allDevices()  error:  "org.freedesktop.DBus.Error.ServiceUnknown"
kf.kirigami: Failed to find a Kirigami platform plugin
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
qt.qpa.clipboard: QXcbClipboard::setMimeData: Cannot set X11 selection owner
[940:1202/124037.203282:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/124116.216875:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
kwin_core: XCB error: 3 (BadWindow), sequence: 48272, resource id: 79691813, major code: 129 (SHAPE), minor code: 6 (Input)
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[940:1202/130410.213701:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[940:1202/130501.947073:ERROR:simple_index_file.cc(322)] Failed to write the temporary index file
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
kwin_core: XCB error: 3 (BadWindow), sequence: 6216, resource id: 6293279, major code: 129 (SHAPE), minor code: 6 (Input)
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'baseline#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'baseline#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'dirtybit' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'prototype-no-code-events#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
org.kde.klipper: Failed to save history. Clipboard history cannot be saved.
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'top-sites#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#start' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab#sequence' into glean_internal_info: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_configured' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'newtab.sov_allocation' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[ERROR glean_core::database] Failed to record metric 'topsites.sponsored_tiles_received' into newtab: Error { kind: Rkv(IoError(Os { code: 122, kind: FilesystemQuotaExceeded, message: "Disk quota exceeded" })) }
[Parent 22573, Unnamed thread 7f72bd0a5ca0] WARNING: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.C74YX2”: Disk quota exceeded: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:201

(firefox:22573): dconf-WARNING **: 14:02:36.309: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.C74YX2”: Disk quota exceeded
[Parent 22573, Main Thread] WARNING: Attempting to store changes into '/afs/mpa/home/basu/.local/share/recently-used.xbel', but failed: Failed to create file “/afs/mpa/home/basu/.local/share/recently-used.xbel.IELZX2”: Disk quota exceeded: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:201

(firefox:22573): Gtk-WARNING **: 14:02:36.312: Attempting to store changes into '/afs/mpa/home/basu/.local/share/recently-used.xbel', but failed: Failed to create file “/afs/mpa/home/basu/.local/share/recently-used.xbel.IELZX2”: Disk quota exceeded
[Parent 22573, Unnamed thread 7f72bd0a5ca0] WARNING: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.QW2VX2”: Disk quota exceeded: 'glib warning', file /builds/worker/checkouts/gecko/toolkit/xre/nsSigHandlers.cpp:201

(firefox:22573): dconf-WARNING **: 14:02:45.739: failed to commit changes to dconf: GDBus.Error:org.gtk.GDBus.UnmappedGError.Quark._g_2dfile_2derror_2dquark.Code24: Failed to create file “/afs/mpa/home/basu/.config/dconf/user.QW2VX2”: Disk quota exceeded

